ED2: Two-stage Active Learning for Error Detection -- Technical Report

Traditional error detection approaches require user-defined parameters and rules. Thus, the user has to know both the error detection system and the data. However, we can also formulate error detection as a semi-supervised classification problem that only requires domain expertise. The challenges for such an approach are twofold: (1) to represent the data in a way that enables a classification model to identify various kinds of data errors, and (2) to pick the most promising data values for learning. In this paper, we address these challenges with ED2, our new example-driven error detection method. First, we present a new two-dimensional multi-classifier sampling strategy for active learning. Second, we propose novel multi-column features. The combined application of these techniques provides fast convergence of the classification task with high detection accuracy. On several real-world datasets, ED2 requires, on average, less than 1% labels to outperform existing error detection approaches. This report extends the peer-reviewed paper "ED2: A Case for Active Learning in Error Detection". All source code related to this project is available on GitHub.

==> charts/features_all/features_address.tex <==
\nextgroupplot[legend to name=testLegendfeatures, 
title={Address},
%ylabel={$F_1$-score},
xmin=0.0, xmax=\limitaddress]
                
%addplot
%\addplot+[mark=none] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(20,0.0)(24,0.0)(28,0.0)(38,0.0)(48,0.0)(58,0.0)(68,0.14240343779747952)(78,0.5741965011024701)(88,0.6522479213872837)(98,0.7754172263354274)(108,0.8348535468119946)(118,0.9201583523198711)(128,0.9467868300437523)(138,0.9557015103847423)(148,0.9699006951278741)(158,0.9746786998563955)(168,0.9762495029966646)(178,0.976545131810877)(188,0.9790016833913986)(198,0.9784384381945717)(208,0.980207552681498)(218,0.9776896583207882)(228,0.9821551159400732)(238,0.9837952497957545)(248,0.9829444718035221)(258,0.9851874777131442)(268,0.9842950322383803)(278,0.9858819102302974)(288,0.986225954973888)(298,0.986627587462511)(308,0.9869414419184146)(318,0.9870350877016698)(328,0.9873929884459466)(338,0.9878255751809604)(348,0.9886482204112863)(358,0.988889526263099)(368,0.9890766571575952)(378,0.9890557075074599)(388,0.9898389569861441)(398,0.9898419789080177)(408,0.9899748656743992)(418,0.9912639400969289)(428,0.991396010646308)(438,0.9915440908783468)(448,0.9920261300132875)(458,0.9921330040192424)(468,0.992160054515851)(478,0.9921668779730888)(488,0.992212602756771)(498,0.9922987806783)};
%\addlegendentry{Char unigrams + Metadata}
%\addplot+[mark=none] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(20,0.0)(24,0.0)(28,0.0)(38,0.0)(48,0.0)(58,0.0)(68,0.19995409243531567)(78,0.6112051102782933)(88,0.7079108933482053)(98,0.8205996556791664)(108,0.8437447761006975)(118,0.9104151579182244)(128,0.9618838920958414)(138,0.9595439739377465)(148,0.9734346709823587)(158,0.97706376384097)(168,0.9776623334222654)(178,0.9790006612833974)(188,0.9766166491091051)(198,0.9816153449360636)(208,0.9826337371514778)(218,0.9855170676919502)(228,0.9817172430181159)(238,0.9847993684204628)(248,0.9869115719174422)(258,0.9873941722941257)(268,0.9873958105606795)(278,0.9869795947316675)(288,0.9883767810191971)(298,0.988414942545259)(308,0.9859568483422322)(318,0.9882110375267381)(328,0.9889320040932562)(338,0.9901150523241762)(348,0.9899610103050789)(358,0.9901495437265758)(368,0.9904605404935071)(378,0.9905098641110378)(388,0.9904988018141851)(398,0.9906324412181962)(408,0.990994007726408)(418,0.991004637269517)(428,0.9910262523885678)(438,0.9910771686350965)(448,0.9912105740558831)(458,0.9912514931138686)(468,0.9912904812016846)(478,0.9912846920439795)(488,0.9913491358969804)(498,0.9913587284027561)};
%\addlegendentry{Char unigrams + Metadata + Error correlation}

%\addplot+[mark=none] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(20,0.0)(24,0.0)(28,0.0)(38,0.0)(48,0.0)(58,0.0)(68,0.02873870203848894)(78,0.5167149752772612)(88,0.5401183664418342)(98,0.6610004463046945)(108,0.7006701186932549)(118,0.8066432482660139)(128,0.9147015577142055)(138,0.9666231229416347)(148,0.9687038714339572)(158,0.9718701531273114)(168,0.9734432557717867)(178,0.9747530164241611)(188,0.9627406446676419)(198,0.9842692244342555)(208,0.9843675593770043)(218,0.986324950867474)(228,0.9865392481707695)(238,0.9870821952947768)(248,0.9855278254607132)(258,0.9851011714888814)(268,0.9875551644103728)(278,0.9875476749222145)(288,0.9879023500073727)(298,0.9875941628791921)(308,0.9892809120506293)(318,0.9898130764107818)(328,0.9898146897438165)(338,0.9899624535721869)(348,0.9901223967556583)(358,0.9901861176156694)(368,0.9902579657421204)(378,0.989883063943874)(388,0.9906692506115057)(398,0.9908215285460221)(408,0.9907751329383615)(418,0.9909574899088105)(428,0.9909300755285593)(438,0.9910791957388299)(448,0.991281200956075)(458,0.9914359681012807)(468,0.9918588890398354)(478,0.9919270773047837)(488,0.9919395203433062)(498,0.9920969242591212)};
%\addlegendentry{LSTM + Metadata}


\addplot+[mark=none] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(20,0.0)(24,0.0)(28,0.0)(38,0.0)(48,0.0)(58,0.0)(68,0.050560981372710125)(78,0.3713195128604468)(88,0.4036529210468454)(98,0.5567434739668784)(108,0.6245133197573592)(118,0.6866625575257236)(128,0.7331976115132591)(138,0.80465630516502)(148,0.8724968636614976)(158,0.8888891004703087)(168,0.90205909537417)(178,0.9117367082912089)(188,0.9193152227199283)(198,0.9230434776424236)(208,0.9244346241954229)(218,0.927277587139298)(228,0.9318001073036196)(238,0.9336595442779971)(248,0.9367225528663784)(258,0.9381066663989565)(268,0.9427679152252171)(278,0.9445113197638909)(288,0.9480881542624575)(298,0.9580555615016655)(308,0.9569675539082663)(318,0.961958466209366)(328,0.9679962690253916)(338,0.9683429136072466)(348,0.9688739902915506)(358,0.9700764098632828)(368,0.9717430658631752)(378,0.9720667235220386)(388,0.9712060884298721)(398,0.9715386130361742)(408,0.9730916185086294)(418,0.9737730295960144)(428,0.9737254854275557)(438,0.9735937241284509)(448,0.9746845883553916)(458,0.9755990441621736)(468,0.9760930767354985)(478,0.9765455030523548)(488,0.9772254744907635)(498,0.9777360049666995)};
\addlegendentry{Character-level $\rho_{\text{n-grams}}(n=1)$}



\addplot+[mark=none] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(20,0.0)(24,0.0)(28,0.0)(38,0.0)(48,0.0)(58,0.0)(68,0.05960856613870576)(78,0.40610362000225775)(88,0.43665269922848243)(98,0.5844229997463297)(108,0.6001510551089784)(118,0.6522592932964247)(128,0.7468529581664296)(138,0.7945031071399588)(148,0.8639328716795178)(158,0.8974240846938855)(168,0.9137501329377645)(178,0.920024638030255)(188,0.9250317802237383)(198,0.9296705784463943)(208,0.9310973859658654)(218,0.935178017267958)(228,0.936698163038012)(238,0.943878822856392)(248,0.9561007050981157)(258,0.9589945066185953)(268,0.961482290388781)(278,0.9574911489232031)(288,0.9625097950403039)(298,0.9573059710049066)(308,0.9649569721024474)(318,0.9698149908239395)(328,0.969966219333641)(338,0.97175505473051)(348,0.9729100864825033)(358,0.9744414764174912)(368,0.9763095573668)(378,0.9765295332971217)(388,0.9765177452590234)(398,0.9777850378154291)(408,0.9785828207910647)(418,0.9791121511602539)(428,0.9793166388732324)(438,0.9805361141520743)(448,0.980992040364991)(458,0.9813805621629499)(468,0.9817940287194465)(478,0.9822386717303411)(488,0.9824730021100292)(498,0.9830908242122878)};
\addlegendentry{Character-level $\rho_{\text{n-grams}}(n=2)$}



%\addplot+[mark=none, thick, dash dot] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(20,0.0)(24,0.0)(28,0.0)(38,0.0)(48,0.0)(58,0.0)(68,0.137016111286)(78,0.486418964162)(88,0.566338400104)(98,0.577669110192)(108,0.658338039152)(118,0.733533735755)(128,0.804481928996)(138,0.842591716737)(148,0.876665241424)(158,0.88839377099)(168,0.922406823761)(178,0.929293714832)(188,0.933299448143)(198,0.93985948156)(208,0.952171462241)(218,0.953813124634)(228,0.96056919277)(238,0.963110208841)(248,0.96468420488)(258,0.966436767044)(268,0.963691347229)(278,0.966595048448)(288,0.966728519056)(298,0.969037483352)(308,0.969730977322)(318,0.970223043687)(328,0.973848208219)(338,0.973158778097)(348,0.97487280959)(358,0.974104079639)(368,0.974419751375)(378,0.975542751843)(388,0.975909737274)(398,0.974861727854)(408,0.975746913366)(418,0.976243053613)(428,0.976082774018)(438,0.97665768799)(448,0.977440469028)(458,0.977686388746)(468,0.977783631989)(478,0.977963907482)(488,0.977916085508)(498,0.978126257255)(508,0.978291798118)(518,0.978499484188)(528,0.978729965735)(538,0.978732759366)(548,0.978894790387)(558,0.979032657561)(568,0.979109097746)};
%\addlegendentry{$\rho_{\text{LSTM}}$}


\addplot+[mark=none, thick, dash dot] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(20,0.0)(24,0.0)(28,0.0)(38,0.0)(48,0.0)(58,0.0)(68,0.26399522235378087)(78,0.6466064010045365)(88,0.7802934354483384)(98,0.8768939512544301)(108,0.9220513731471677)(118,0.9493463992609954)(128,0.9543814589486832)(138,0.9553809327997659)(148,0.9627356592414464)(158,0.9627356592414464)(168,0.9647989638860691)(178,0.9595257667052293)(188,0.9760115068793306)(198,0.978871743131012)(208,0.9720815504529317)(218,0.9790204725689386)(228,0.9786652312067321)(238,0.9789630614658604)(248,0.9778217027453844)(258,0.9755456866173224)(268,0.9738200940169097)(278,0.9792252034068334)(288,0.9796695520555015)(298,0.9811633481981434)(308,0.9815016375797774)(318,0.9830743440494037)(328,0.9831176994835127)(338,0.9832212334285357)(348,0.9841197679949426)(358,0.9851729988704634)(368,0.9863258994382894)(378,0.986787605202583)(388,0.9874663630822059)(398,0.9875981555486286)(408,0.9878096836211586)(418,0.9874907977297926)(428,0.98795984431944)(438,0.9881628544656426)(448,0.9882821367243168)(458,0.9887179036387364)(468,0.9888376058238724)(478,0.9891471993243692)(488,0.9886054010829005)(498,0.989117205142421)};
\addlegendentry{$\rho_{\text{meta}}$}
\addplot+[mark=none] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(20,0.0)(24,0.0)(28,0.0)(38,0.0)(48,0.0)(58,0.0)(68,0.0)(78,0.4347642712481564)(88,0.4347642712481564)(98,0.4528387046373327)(108,0.44965327490259094)(118,0.44965327490259094)(128,0.44965327490259094)(138,0.46846076094365746)(148,0.46792939715669907)(158,0.46792939715669907)(168,0.5733632988652673)(178,0.578965919728121)(188,0.5877845442314507)(198,0.5870411544474433)(208,0.5872227376718065)(218,0.5892181477419595)(228,0.5873377651156002)(238,0.5878268637322578)(248,0.5901341579776448)(258,0.5957593752397168)(268,0.5973365431705696)(278,0.6101686653018098)(288,0.6106422778593582)(298,0.6126070076883262)(308,0.6180528110997607)(318,0.600753188030395)(328,0.5971841031094983)(338,0.5959683759100101)(348,0.6404215747056902)(358,0.6449048563208183)(368,0.6513742142876018)(378,0.6615428254152175)(388,0.6757489200799714)(398,0.6770167696380003)(408,0.6785246604382834)(418,0.6741818332010514)(428,0.6743192296538782)(438,0.6749201325471309)(448,0.6793486161502599)(458,0.6782556359032703)(468,0.6780412547181902)(478,0.6787219977967041)(488,0.6822513872986781)(498,0.6845847395859458)};
\addlegendentry{Word-level $\rho_{\text{n-grams}}(n=1)$}

\addplot+[mark=none] coordinates{(4,0.000111408642923)(8,0.00104156721146)(12,0.00384144165441)(16,0.142226880925)(20,0.294728669591)(24,0.369082681637)(28,0.384307659549)(38,0.434406805219)(48,0.499055764767)(58,0.584660595794)(68,0.544884838424)(78,0.490643012131)(88,0.378027538264)(98,0.362161916069)(108,0.396732102726)(118,0.431575034692)(128,0.452373091849)(138,0.470192717745)(148,0.507096201693)(158,0.543081127208)(168,0.585604175691)(178,0.618684078979)(188,0.637979998882)(198,0.673649229892)(208,0.70460600068)(218,0.733013387921)(228,0.754185848963)(238,0.7740271568)(248,0.78484957607)(258,0.808163483977)(268,0.818801981041)(278,0.831004007408)(288,0.841980439067)(298,0.847381955178)(308,0.850082458826)(318,0.854234317203)(328,0.858000216059)(338,0.862733837375)(348,0.863107767399)(358,0.8633202745)(368,0.865692400825)(378,0.867079840315)(388,0.867328612453)(398,0.868978622109)(408,0.869281783249)(418,0.870822510491)(428,0.871480389743)(438,0.873438090289)(448,0.874814116147)(458,0.874170980405)(468,0.877665091153)(478,0.878547074211)(488,0.879869275117)(498,0.881624643691)(508,0.881982352091)(518,0.882422808256)(528,0.882937847148)(538,0.883259495097)(548,0.88414903212)(558,0.884360999468)(568,0.884950853497)};
\addlegendentry{$\rho_{\text{w2v}}$}

\addplot+[mark=none] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(20,0.0)(24,0.0)(28,0.0)(38,0.0)(48,0.0)(58,7.6416085837e-06)(68,0.30116256767)(78,0.629540776091)(88,0.763046387279)(98,0.818664936932)(108,0.867090432628)(118,0.888062069709)(128,0.922081186103)(138,0.948045457846)(148,0.961518993742)(158,0.970939997074)(168,0.968627678483)(178,0.971598875458)(188,0.973005809753)(198,0.966708096959)(208,0.976182676404)(218,0.985952985125)(228,0.982805020308)(238,0.987368330221)(248,0.988351338069)(258,0.988470922497)(268,0.989044990785)(278,0.989925754344)(288,0.990438173962)(298,0.99081309716)(308,0.990881195863)(318,0.990883956479)(328,0.990961364614)(338,0.990983338758)(348,0.991095887545)(358,0.991039942894)(368,0.990717764125)(378,0.991662124539)(388,0.991450790375)(398,0.991591945496)(408,0.991997842939)(418,0.992106367922)(428,0.992142984531)(438,0.992117394319)(448,0.992213246493)(458,0.99223100926)(468,0.992278687565)(478,0.99264164399)(488,0.992796037811)(498,0.992832910049)(508,0.992874625375)(518,0.992865649037)(528,0.992995267785)(538,0.993041182036)(548,0.993164651404)(558,0.993242641765)(568,0.99334677101)};
\addlegendentry{$\rho_{\text{\system}} \setminus \{ \rho_{\text{error}}\}$}

\addplot+[mark=none, black] coordinates{(4,5.57043214617e-05)(8,0.000770131313035)(12,0.00258981673248)(16,0.0761495003703)(20,0.175006337204)(24,0.264270158576)(28,0.300285413506)(38,0.334525872174)(48,0.37960710205)(58,0.419816516404)(68,0.393184072361)(78,0.574541660862)(88,0.531939168201)(98,0.683455776853)(108,0.75991041799)(118,0.835520570216)(128,0.901719664236)(138,0.954807818214)(148,0.974378773945)(158,0.976456412918)(168,0.977810099187)(178,0.977526223595)(188,0.977789784894)(198,0.97918458833)(208,0.979005029974)(218,0.979850247544)(228,0.983238043903)(238,0.985393627225)(248,0.976763947524)(258,0.98544140125)(268,0.985280201349)(278,0.985829274018)(288,0.986500154704)(298,0.987617837884)(308,0.983155114088)(318,0.984627938379)(328,0.986972726229)(338,0.988813264942)(348,0.988060586867)(358,0.988062203895)(368,0.98879832559)(378,0.988854496017)(388,0.98867251495)(398,0.989645033356)(408,0.989787060881)(418,0.989979834727)(428,0.990023853161)(438,0.99013276516)(448,0.990263165219)(458,0.990112714178)(468,0.990322009701)(478,0.990324897267)(488,0.990435445146)(498,0.991137663201)(508,0.991570978924)(518,0.991715991982)(528,0.992076573078)(538,0.992520205565)(548,0.9925814222)(558,0.993223067917)(568,0.993228192589)};
\addlegendentry{$\rho_{\text{\system}}$}





==> charts/features_all/features_beers.tex <==
\nextgroupplot[title={Beers},
%ylabel={$F_1$-score},
xmin=0.0, xmax=\limitbeers]
                
%\addplot+[mark=none] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(26,0.400337699602)(36,0.410291338225)(46,0.408910594888)(56,0.410034778399)(66,0.568729180092)(76,0.736895590238)(86,0.827769776652)(96,0.918813903645)(106,0.946718720894)(116,0.947688986039)(126,0.948334188912)(136,0.95025035031)(146,0.950889987198)(156,0.953801282692)(166,0.954535415944)(176,0.958169459563)(186,0.961242677869)(196,0.961242677869)(206,0.965576914841)(216,0.965631560571)(226,0.970263824515)(236,0.972071839026)(246,0.973950698674)(256,0.974083580216)(266,0.978798895319)(276,0.978798895319)(286,0.981837846483)(296,0.983591384609)(306,0.98446993758)(316,0.984823730516)(326,0.988054199835)(336,0.992947841107)(346,0.993828658724)(356,0.993828658724)(366,0.993956896734)(376,0.993956896734)(386,0.994335601466)(396,0.996005856714)(406,0.99680791913)(416,0.997425118234)(426,1.0)(436,1.0)(446,1.0)};
%\addlegendentry{Char unigrams + Metadata}


%\addplot+[mark=none] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(26,0.396808461533)(36,0.402384641763)(46,0.401157575721)(56,0.402135635874)(66,0.531778941551)(76,0.791787738639)(86,0.899034583912)(96,0.916434984205)(106,0.925184820408)(116,0.942259256703)(126,0.942528229987)(136,0.942720883044)(146,0.944358814259)(156,0.944420783223)(166,0.955201938499)(176,0.961430214087)(186,0.964580813628)(196,0.964580813628)(206,0.964798934902)(216,0.964798934902)(226,0.96775131064)(236,0.972277851571)(246,0.976338912048)(256,0.982892625498)(266,0.98471839493)(276,0.985026719699)(286,0.985026719699)(296,0.993681917211)(306,0.9960873037)(316,0.996610169492)(326,0.99987176199)(336,0.99987176199)(346,0.99987176199)(356,0.99987176199)(366,1.0)(376,0.999588477366)(386,1.0)(396,1.0)(406,1.0)(416,1.0)(426,1.0)(436,1.0)(446,1.0)};
%\addlegendentry{Char unigrams + Metadata + Error correlation}


%\addplot+[mark=none] coordinates{(4,0.0)};
%\addlegendentry{LSTM + Metadata}


\addplot+[mark=none] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(26,0.297857382098)(36,0.300852345282)(46,0.302165633962)(56,0.303001669221)(66,0.459472654764)(76,0.476641660026)(86,0.476964575959)(96,0.481903117353)(106,0.530990005449)(116,0.538763487278)(126,0.635738895918)(136,0.759997769849)(146,0.818368790464)(156,0.839796266744)(166,0.879047044501)(176,0.913644462028)(186,0.930883958514)(196,0.931837965967)(206,0.931804951355)(216,0.931743604357)(226,0.932142591651)(236,0.932175262686)(246,0.933427913035)(256,0.933457078825)(266,0.933961745365)(276,0.935049903307)(286,0.935049903307)(296,0.935158794586)(306,0.935589065709)(316,0.935646639087)(326,0.935643232257)(336,0.936684325072)(346,0.936693019945)(356,0.937118969287)(366,0.937854053836)(376,0.93798102552)(386,0.938221826264)(396,0.938221826264)(406,0.938289864598)(416,0.939228783424)(426,0.940020476216)(436,0.941560216459)(446,0.942076104044)};
%\addlegendentry{Char unigrams}


\addplot+[mark=none] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(26,0.268073179442)(36,0.273988383231)(46,0.275409237998)(56,0.275977818845)(66,0.445386221647)(76,0.462240113568)(86,0.464363098433)(96,0.504861347897)(106,0.534161871451)(116,0.54435841364)(126,0.634280699943)(136,0.747142252807)(146,0.824634320638)(156,0.886303697497)(166,0.928256050727)(176,0.932868980633)(186,0.933076433795)(196,0.93316402992)(206,0.93309105256)(216,0.934166711582)(226,0.934619607383)(236,0.934772279059)(246,0.934529835887)(256,0.935104571774)(266,0.935183644457)(276,0.935208918994)(286,0.935402606507)(296,0.936440727189)(306,0.936288060949)(316,0.936949403106)(326,0.936974897051)(336,0.936974897051)(346,0.937989249545)(356,0.937989249545)(366,0.937970445345)(376,0.938480221496)(386,0.93881952828)(396,0.93949246953)(406,0.940176015755)(416,0.940598463601)(426,0.94095697626)(436,0.941072315284)(446,0.941231974677)};
%\addlegendentry{Char bigrams}

%\addplot+[mark=none] coordinates{(4,0.0)};
%\addlegendentry{$\rho_{\text{LSTM}}$}


\addplot+[mark=none, thick, dash dot] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(26,0.414685488497)(36,0.56522051095)(46,0.564750043573)(56,0.567194413021)(66,0.837312165269)(76,0.892038815883)(86,0.900070885639)(96,0.912442975079)(106,0.9095917386)(116,0.909543463759)(126,0.910095013996)(136,0.919673331821)(146,0.922511243477)(156,0.946252825928)(166,0.957491173985)(176,0.961549824345)(186,0.965523297879)(196,0.9653329999)(206,0.966691071937)(216,0.96797626897)(226,0.96832724254)(236,0.972170831324)(246,0.979558734481)(256,0.981673979019)(266,0.983480751092)(276,0.983964691215)(286,0.985377896153)(296,0.9865041819)(306,0.988467309387)(316,0.992577022892)(326,0.992654072118)(336,0.992783745896)(346,0.992783745896)(356,0.993169515657)(366,0.997532468875)(376,0.999149994161)(386,0.999846403221)(396,0.999846403221)(406,0.999872024538)(416,0.999872024538)(426,0.999948770488)(436,0.999948770488)(446,0.999948770488)};
%\addlegendentry{Metadata}


\addplot+[mark=none] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(26,0.140198072158)(36,0.162224779347)(46,0.15890888412)(56,0.158867873331)(66,0.16858499163)(76,0.175760925557)(86,0.176487693079)(96,0.185535191584)(106,0.18584355763)(116,0.178583498547)(126,0.183200296336)(136,0.187856290005)(146,0.186181613047)(156,0.177714287867)(166,0.163571075427)(176,0.161385154289)(186,0.157020631101)(196,0.155443722885)(206,0.151984352075)(216,0.153966216386)(226,0.156077949285)(236,0.155326113675)(246,0.151312149527)(256,0.151072910666)(266,0.14979773159)(276,0.144735767374)(286,0.147551079858)(296,0.149075259475)(306,0.148260171736)(316,0.150239249906)(326,0.148528420972)(336,0.147562689599)(346,0.146691100807)(356,0.146272709358)(366,0.143775193801)(376,0.141888520466)(386,0.142303813734)(396,0.142700314123)(406,0.142506105837)(416,0.143043869091)(426,0.145735213166)(436,0.146328207382)(446,0.146382937691)};
%\addlegendentry{Word unigrams}


\addplot+[mark=none] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(26,0.105763109628)(36,0.115280290318)(46,0.117913684024)(56,0.118864731339)(66,0.327862711302)(76,0.395845332699)(86,0.467166792373)(96,0.552534381155)(106,0.682580237472)(116,0.704801891426)(126,0.711894527233)(136,0.770047821917)(146,0.783254850229)(156,0.797768341575)(166,0.803459643519)(176,0.817866123631)(186,0.832545672524)(196,0.838636183936)(206,0.843844394574)(216,0.8486966564)(226,0.854871637219)(236,0.860036390816)(246,0.869802675621)(256,0.874821068183)(266,0.882737261547)(276,0.888966103519)(286,0.89186066344)(296,0.897358486332)(306,0.903069144419)(316,0.905234999895)(326,0.908252652966)(336,0.913902151327)(346,0.916428869048)(356,0.917701527234)(366,0.919178221744)(376,0.922506073343)(386,0.923945292292)(396,0.927460792115)(406,0.930900050599)(416,0.934266053265)(426,0.938051355615)(436,0.939054318061)(446,0.940965847875)};
%\addlegendentry{Word2Vec}

\addplot+[mark=none] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(26,0.229329637273)(36,0.234305778538)(46,0.235683801414)(56,0.237115631792)(66,0.55893146095)(76,0.773701464014)(86,0.855615266456)(96,0.921719096118)(106,0.950148865928)(116,0.950376477526)(126,0.95626525723)(136,0.957387212461)(146,0.957332146233)(156,0.961914204507)(166,0.964768306706)(176,0.965926737435)(186,0.970023536696)(196,0.976054425958)(206,0.976244828893)(216,0.97729456999)(226,0.980575080044)(236,0.983228175495)(246,0.983282879097)(256,0.983282879097)(266,0.983282879097)(276,0.98556601691)(286,0.98556601691)(296,0.986262431664)(306,0.987906198587)(316,0.993466440174)(326,0.99390242407)(336,0.996992084433)(346,0.996992084433)(356,0.996992084433)(366,0.996992084433)(376,0.996992084433)(386,0.996992084433)(396,0.996992084433)(406,0.996992084433)(416,0.999459181046)(426,1.0)(436,1.0)(446,1.0)};
%\addlegendentry{Char unigrams + Metadata+ Word2Vec}

\addplot+[mark=none, black] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(26,0.355747523108)(36,0.360915294744)(46,0.364017758745)(56,0.365024225466)(66,0.513546779872)(76,0.788256936715)(86,0.875355126852)(96,0.943880453182)(106,0.944558037082)(116,0.944786389388)(126,0.944874132476)(136,0.950390766524)(146,0.950450874548)(156,0.95081143732)(166,0.959296600138)(176,0.965375894461)(186,0.968738351438)(196,0.973957211721)(206,0.976757402121)(216,0.979273600257)(226,0.98076467162)(236,0.986352826695)(246,0.989633249975)(256,0.990976771431)(266,0.990976771431)(276,0.993830682963)(286,0.996774193548)(296,0.996774193548)(306,0.996774193548)(316,0.996774193548)(326,0.997127799736)(336,1.0)(346,1.0)(356,1.0)(366,1.0)(376,1.0)(386,1.0)(396,1.0)(406,1.0)(416,1.0)(426,1.0)(436,1.0)(446,1.0)};
%\addlegendentry{Char unigrams + Metadata + Error correlation + Word2Vec}





==> charts/features_all/features_flights.tex <==
\nextgroupplot[title={Flights},
ylabel={$F_1$-score},
xmin=0.0, xmax=\limitflights]


                

%\addplot+[mark=none] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(26,0.3009828033510852)(36,0.5261875013216127)(46,0.6574735566846837)(56,0.7838476062023378)(66,0.7889281216279175)(76,0.7966459938487097)(86,0.8155764784363694)(96,0.8340225045292667)(106,0.8467671035322368)(116,0.861908390684745)(126,0.87429555337602)(136,0.8814245695785825)(146,0.8880835123925991)(156,0.8926581255143615)(166,0.8976074732499342)(176,0.9024917129518293)(186,0.9081079570444335)(196,0.9118599009653838)(206,0.9173633562596045)(216,0.9202480039563478)(226,0.9232285636775994)(236,0.9243026199361546)(246,0.9281721415287523)(256,0.9329826853990767)};
%\addlegendentry{Char unigrams + Metadata}
%\addplot+[mark=none] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(26,0.30180848911197244)(36,0.5391035461086628)(46,0.6797768636644462)(56,0.795873699528614)(66,0.8081525233107758)(76,0.8225421879593127)(86,0.8288507293779318)(96,0.8412962983648938)(106,0.8468428196691556)(116,0.8546241135230728)(126,0.8691026491643079)(136,0.8767119896306653)(146,0.8841295011606671)(156,0.8894012598068274)(166,0.8939248390735928)(176,0.8987651923697924)(186,0.9044897040048054)(196,0.9090145540144015)(206,0.9109234404976443)(216,0.9110008819327575)(226,0.9153995381959843)(236,0.9183742955185048)(246,0.9205879669103038)(256,0.9237649187234132)};
%\addlegendentry{Char unigrams + Metadata + Error correlation}

%\addplot+[mark=none] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(26,0.29945755019900877)(36,0.5715822712586903)(46,0.6795516708737666)(56,0.7765193490075755)(66,0.7855227727742078)(76,0.8035217743914951)(86,0.8140165748232773)(96,0.8307389678882597)(106,0.8377875565913471)(116,0.8424763023295068)(126,0.8471441081543851)(136,0.8566980171480768)(146,0.8657140653114137)(156,0.8766048650996577)(166,0.8843452372587933)(176,0.8918452642303194)(186,0.8976074173903668)(196,0.902075301979257)(206,0.9072303152726503)(216,0.9113924704195455)(226,0.9159920297213479)(236,0.9209297298583161)(246,0.9245456525341252)(256,0.9284747950046119)};
%\addlegendentry{LSTM + Metadata}



\addplot+[mark=none] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(26,0.3024153914981233)(36,0.5282507980398206)(46,0.654907745648127)(56,0.7618137091175938)(66,0.7724794546598005)(76,0.7929338489620101)(86,0.7960828537233899)(96,0.7975094745482882)(106,0.8105125215239477)(116,0.8162115230788982)(126,0.8180440156261056)(136,0.8321093399976436)(146,0.8348519034915686)(156,0.8432206371360994)(166,0.8512232652701792)(176,0.860025147431349)(186,0.8663084273044674)(196,0.8710238308239043)(206,0.877088548421112)(216,0.8806314216918372)(226,0.8850590628183328)(236,0.8876496969491235)(246,0.892387993652593)(256,0.8971066222406746)};
%\addlegendentry{Char unigrams}
\addplot+[mark=none] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(26,0.3013375274760782)(36,0.5522097205069343)(46,0.6364259905846315)(56,0.7435665396956544)(66,0.7681262006039427)(76,0.7803869190996756)(86,0.8030577290328852)(96,0.8137517304092661)(106,0.824145618605334)(116,0.8307897378944423)(126,0.8373959261609072)(136,0.8465077985790088)(146,0.8567281642972342)(156,0.860291529264634)(166,0.8659083051726981)(176,0.8720219846669404)(186,0.8772507827566134)(196,0.8806750748700333)(206,0.8873619636323591)(216,0.8907092978010629)(226,0.8955954555732175)(236,0.9005559999354382)(246,0.903117299338289)(256,0.906141767431458)};
%\addlegendentry{Char bigrams}

%\addplot+[mark=none, thick, dash dot] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(26,0.122578615733)(36,0.452095976696)(46,0.593146165478)(56,0.694710476595)(66,0.712595697457)(76,0.726983773802)(86,0.751901241032)(96,0.775827756489)(106,0.82463827283)(116,0.829790605568)(126,0.838547899306)(136,0.846174236412)(146,0.854435734701)(156,0.857015236887)(166,0.864319624729)(176,0.86497684225)(186,0.869334402532)(196,0.87425698046)(206,0.879072510134)(216,0.884154353151)(226,0.887667450896)(236,0.894428654289)(246,0.901635075949)(256,0.906575863528)(266,0.910708838147)(276,0.913859346008)(286,0.919644701703)};
%\addlegendentry{$\rho_{\text{LSTM}}$}

\addplot+[mark=none, thick, dash dot] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(26,0.24976955733563333)(36,0.4967271008673439)(46,0.5937318870895656)(56,0.7037294337372246)(66,0.7369213064356505)(76,0.7526716624310102)(86,0.7601880284189925)(96,0.7781571167164343)(106,0.7954399306314219)(116,0.8103041325851941)(126,0.8263340686758273)(136,0.8312914735134745)(146,0.8482281429008767)(156,0.8573832453306034)(166,0.8647563638801987)(176,0.8727470967588934)(186,0.8795746818979675)(196,0.8845788178329593)(206,0.8905556149679906)(216,0.8965191677270763)(226,0.9012687770152192)(236,0.9044478323036955)(246,0.9062776590463709)(256,0.9078811796462158)};
%\addlegendentry{Metadata}
\addplot+[mark=none] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(26,0.029234209974951703)(36,0.1443012790310494)(46,0.21093901863397652)(56,0.2710581359612952)(66,0.3238181973314972)(76,0.3395624050445677)(86,0.3799912637979062)(96,0.3990307961895736)(106,0.4127533598037137)(116,0.4377293547890685)(126,0.44368700924027527)(136,0.46417499372212995)(146,0.4836553941199441)(156,0.49603861969553986)(166,0.5119120167782885)(176,0.5150851595806858)(186,0.5204194776254921)(196,0.5286948669113747)(206,0.5401335214371052)(216,0.5472706536977572)(226,0.5493751913542344)(236,0.5529925247972459)(246,0.5538614452426824)(256,0.5577187412814919)};
%\addlegendentry{Word unigrams}


\addplot+[mark=none] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(26,0.274573357484)(36,0.540838348082)(46,0.651522516818)(56,0.76034809952)(66,0.77318712978)(76,0.786213818666)(86,0.801449910334)(96,0.808180302093)(106,0.820052209786)(116,0.829049480665)(126,0.837442406302)(136,0.844487192293)(146,0.858747176088)(156,0.862163166885)(166,0.870052844642)(176,0.873947485717)(186,0.876717712434)(196,0.886218436499)(206,0.891707743608)(216,0.896905785504)(226,0.901550325518)(236,0.904964065523)(246,0.905961371983)(256,0.911044538917)(266,0.915218963454)(276,0.919541208725)(286,0.923784827753)};
%\addlegendentry{Word2Vec}


\addplot+[mark=none] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(26,0.146042432383)(36,0.419174308658)(46,0.526061017642)(56,0.652082838724)(66,0.682377876858)(76,0.718387939499)(86,0.757679802998)(96,0.786867524649)(106,0.811865899999)(116,0.834284882457)(126,0.843511784381)(136,0.860391546576)(146,0.87752313163)(156,0.883937115638)(166,0.893001841251)(176,0.903294548374)(186,0.910210896871)(196,0.914933613192)(206,0.922202490171)(216,0.926254121531)(226,0.931971157113)(236,0.935913770075)(246,0.938559030116)(256,0.943513958035)(266,0.945687885)(276,0.949192311191)(286,0.952495739739)};
%\addlegendentry{Char unigrams + Metadata + Word2Vec}

\addplot+[mark=none, black] coordinates{(4,0.174808114035)(8,0.295762455923)(12,0.396196265773)(16,0.488310733565)(26,0.593472088167)(36,0.686717721195)(46,0.734377258196)(56,0.787735034815)(66,0.807734607929)(76,0.822575395328)(86,0.83269145929)(96,0.846267222307)(106,0.86054513197)(116,0.871938396169)(126,0.881360293616)(136,0.886764005995)(146,0.894667172177)(156,0.906847993689)(166,0.910121065962)(176,0.915354155589)(186,0.918875753539)(196,0.924078738366)(206,0.927862461545)(216,0.932168248625)(226,0.935302616591)(236,0.940198595218)(246,0.941935833797)(256,0.943772821041)(266,0.945489556424)(276,0.948097400636)(286,0.948780246342)};
%\addlegendentry{Char unigrams + Metadata + Error correlation + Word2Vec}



                



==> charts/features_all/features_movies.tex <==
\nextgroupplot[title={Movies},
%ylabel={$F_1$-score},
xmin=0.0, xmax=\limitmovies]
                
%\addplot+[mark=none] coordinates{(4,0.0170959397143)(8,0.0130497365085)(12,0.0335584948719)(16,0.0381578998364)(20,0.0335890246455)(24,0.0333601940649)(28,0.0358857103899)(32,0.0370717186216)(36,0.0376667048624)(40,0.0384800561493)(50,0.0374832325759)(60,0.0416314785342)(70,0.0388401568922)(80,0.0350379910704)(90,0.0398925767654)(100,0.0405347928958)(110,0.0340839890769)(120,0.0248341019008)(130,0.0126869868406)(140,0.0)(150,0.134459746663)(160,0.178426078494)(170,0.220204215858)(180,0.270848873775)(190,0.324862932929)(200,0.363090719139)(210,0.416367572446)(220,0.480514088626)(230,0.533822313391)(240,0.574856986974)(250,0.634528778156)(260,0.699044388247)(270,0.750264877273)(280,0.789830072242)(290,0.846878655312)(300,0.869889170046)(310,0.894608859475)(320,0.915738859313)(330,0.918374010468)(340,0.930100992557)(350,0.931367347725)(360,0.932046613393)(370,0.937023662923)(380,0.944368794679)(390,0.945082286025)(400,0.946820560495)(410,0.948926986842)(420,0.948926986842)(430,0.951643696216)(440,0.951575103764)(450,0.951081746117)(460,0.952895583641)(470,0.954102118827)(480,0.942820691998)(490,0.955871640767)(500,0.956947574013)(510,0.956003418695)(520,0.957295035355)(530,0.956829358887)(540,0.957153291256)(550,0.957709550507)(560,0.957805478316)(570,0.958196914017)(580,0.958624231)(590,0.959546429432)(600,0.959770784985)(610,0.96015100282)(620,0.96053393503)(630,0.962653836442)(640,0.963536679096)(650,0.963735225587)(660,0.963927278604)(670,0.964851913046)(680,0.965107546965)(690,0.965721708232)(700,0.965921859937)(710,0.966390840438)(720,0.966929795155)(730,0.966929795155)(740,0.966961699426)(750,0.967341276871)(760,0.968256000542)(770,0.969042288204)(780,0.969293657743)(790,0.969913874108)(800,0.970366876356)(810,0.970462069832)(820,0.970458460778)};
%\addlegendentry{Char unigrams + Metadata}


%\addplot+[mark=none] coordinates{(4,0.0256439095715)(8,0.019484153608)(12,0.0267300447658)(16,0.0318155037526)(20,0.0280402653373)(24,0.0301028407127)(28,0.0323766138183)(32,0.0352252236197)(36,0.0372094728205)(40,0.0383436271937)(50,0.0357693302786)(60,0.0404206432184)(70,0.0392971777801)(80,0.0386828611023)(90,0.0424259591092)(100,0.040697477656)(110,0.0358014495124)(120,0.034458538043)(130,0.0211449780677)(140,0.0)(150,0.142179659024)(160,0.222894401048)(170,0.287626281113)(180,0.311122932349)(190,0.345797182232)(200,0.386885133837)(210,0.410469139957)(220,0.451053316253)(230,0.473091046335)(240,0.48819367549)(250,0.571726590266)(260,0.609759102139)(270,0.702064759995)(280,0.752201547933)(290,0.788755750483)(300,0.827228263421)(310,0.864927081686)(320,0.872723228324)(330,0.895070909392)(340,0.909918811095)(350,0.926991562987)(360,0.928541407779)(370,0.937191626758)(380,0.939254655633)(390,0.941759013223)(400,0.942579889144)(410,0.945135761122)(420,0.945389372041)(430,0.946227308769)(440,0.946335097523)(450,0.950226287196)(460,0.950692181073)(470,0.953217459664)(480,0.955017996212)(490,0.955767856779)(500,0.95792372892)(510,0.958442589946)(520,0.958442589946)(530,0.958401849303)(540,0.958401849303)(550,0.9606089129)(560,0.962224877422)(570,0.962442194011)(580,0.954382896209)(590,0.963410660831)(600,0.963549197925)(610,0.964174636348)(620,0.964148247218)(630,0.964276222594)(640,0.964609996495)(650,0.965364718168)(660,0.965867036059)(670,0.966065680534)(680,0.966736262628)(690,0.967041591837)(700,0.967814371923)(710,0.969180396408)(720,0.969590076807)(730,0.969844402641)(740,0.970151100436)(750,0.970702070734)(760,0.970614629218)(770,0.970647118956)(780,0.971526382433)(790,0.971406095548)(800,0.97216887577)(810,0.972702882798)(820,0.973090932328)};
%\addlegendentry{Char unigrams + Metadata + Error correlation}


%\addplot+[mark=none] coordinates{(4,0.0)};
%\addlegendentry{LSTM + Metadata}


\addplot+[mark=none] coordinates{(4,0.0128219547857)(8,0.0101244859818)(12,0.0331642381546)(16,0.0331642381546)(20,0.0279927844762)(24,0.0284847496005)(28,0.0316318763778)(32,0.0347319038695)(36,0.0352089707634)(40,0.0369068486797)(50,0.0360227093368)(60,0.0384570616155)(70,0.0356393690142)(80,0.0356393690142)(90,0.043371987695)(100,0.0449936818694)(110,0.0389522261818)(120,0.0292430547745)(130,0.0211449780677)(140,0.0)(150,0.112576617626)(160,0.145656531302)(170,0.165414771201)(180,0.207412507667)(190,0.247762568427)(200,0.315270188597)(210,0.362945720162)(220,0.454604145575)(230,0.499069913202)(240,0.549715937993)(250,0.640758805178)(260,0.676288432441)(270,0.741172139807)(280,0.774220894184)(290,0.797825096707)(300,0.837893955816)(310,0.872265990401)(320,0.887803873104)(330,0.895377031794)(340,0.898035600404)(350,0.902788987151)(360,0.912238452015)(370,0.912362307018)(380,0.91971815492)(390,0.922748314095)(400,0.923933800438)(410,0.932094155663)(420,0.937678536946)(430,0.938972279214)(440,0.941539296426)(450,0.943062461386)(460,0.950939547728)(470,0.951522697646)(480,0.954808912479)(490,0.955253309729)(500,0.955966132056)(510,0.956095305474)(520,0.957225872547)(530,0.957705733175)(540,0.958223017896)(550,0.958570184743)(560,0.959701722583)(570,0.95976063326)(580,0.959862218547)(590,0.96016047472)(600,0.960662500381)(610,0.960657766846)(620,0.956881682879)(630,0.962145113826)(640,0.962634003958)(650,0.958570443958)(660,0.964001606206)(670,0.963278732034)(680,0.964626206817)(690,0.96475238772)(700,0.96499004666)(710,0.96531411676)(720,0.965377769589)(730,0.96577926042)(740,0.965947679664)(750,0.966355024799)(760,0.9663888208)(770,0.966547606068)(780,0.966739936297)(790,0.966773735507)(800,0.967197968856)(810,0.967489122482)(820,0.968126900589)};
%\addlegendentry{Char unigrams}


\addplot+[mark=none] coordinates{(4,0.0170959397143)(8,0.0138145548641)(12,0.0189468932643)(16,0.0274296024532)(20,0.0230756967639)(24,0.0262016809945)(28,0.0277723538798)(32,0.0301997541197)(36,0.0319670576935)(40,0.0338110799426)(50,0.0322783126742)(60,0.0383917637996)(70,0.0372547202337)(80,0.0340855931351)(90,0.0381649075694)(100,0.040059185976)(110,0.0391519438125)(120,0.0257772388787)(130,0.0211449780677)(140,0.0)(150,0.103975489667)(160,0.185058971671)(170,0.219651053485)(180,0.266457516908)(190,0.33017796837)(200,0.414685086367)(210,0.473665964029)(220,0.537109808007)(230,0.59072257247)(240,0.657748869764)(250,0.718395630682)(260,0.742410829584)(270,0.792735051595)(280,0.807324403247)(290,0.838936341341)(300,0.85394219168)(310,0.869984387099)(320,0.889347212632)(330,0.896967832474)(340,0.91294296585)(350,0.92213636024)(360,0.92937208021)(370,0.933989745603)(380,0.934057954605)(390,0.944059598911)(400,0.94395623815)(410,0.944166681297)(420,0.945199667022)(430,0.946554216243)(440,0.949151099317)(450,0.951834433567)(460,0.952709983389)(470,0.95348445239)(480,0.953624992112)(490,0.953875013589)(500,0.955260935487)(510,0.955624090757)(520,0.956823450469)(530,0.957851442043)(540,0.95876259843)(550,0.958641250139)(560,0.959720031867)(570,0.953952640916)(580,0.960552707667)(590,0.961395849905)(600,0.961395849905)(610,0.961795276505)(620,0.961861681092)(630,0.961897309172)(640,0.962681831441)(650,0.962774079652)(660,0.96345694418)(670,0.963851063421)(680,0.964777304741)(690,0.965029278587)(700,0.965236834512)(710,0.965436008244)(720,0.965792755215)(730,0.966197466983)(740,0.966474040851)(750,0.966680033266)(760,0.967444848425)(770,0.968049618118)(780,0.968997940771)(790,0.970073350618)(800,0.970277267578)(810,0.970309598171)(820,0.970578150498)};
%\addlegendentry{Char bigrams}


%\addplot+[mark=none] coordinates{(4,0.0)};
%\addlegendentry{$\rho_{\text{LSTM}}$}


\addplot+[mark=none, thick, dash dot] coordinates{(4,0.0213699246429)(8,0.0207860085966)(12,0.0284259327608)(16,0.0329739710158)(20,0.03071001637)(24,0.0299683967735)(28,0.0359308112383)(32,0.0364843048279)(36,0.0377794231253)(40,0.0388181540051)(50,0.0375232376909)(60,0.0404022571479)(70,0.0397181986674)(80,0.0356521263646)(90,0.0371343013804)(100,0.0354594955231)(110,0.0309424894672)(120,0.0296463199719)(130,0.0169159824542)(140,0.0)(150,0.199654884211)(160,0.317892684999)(170,0.400509751119)(180,0.480239114996)(190,0.52523680522)(200,0.558950747385)(210,0.619385823088)(220,0.670079127584)(230,0.70032070332)(240,0.727021603271)(250,0.743125244955)(260,0.760095215997)(270,0.769186603886)(280,0.787543116803)(290,0.796483658381)(300,0.812100751351)(310,0.823515864079)(320,0.831037416074)(330,0.839528263634)(340,0.862450834906)(350,0.870225383899)(360,0.864547408435)(370,0.88430857801)(380,0.897290461608)(390,0.907918910756)(400,0.913642052178)(410,0.927905998148)(420,0.932925658129)(430,0.937757320279)(440,0.934562408528)(450,0.936853017608)(460,0.936029196031)(470,0.939523856354)(480,0.94264435627)(490,0.942573287601)(500,0.942988281854)(510,0.954509800853)(520,0.954799335878)(530,0.951610756509)(540,0.956486553896)(550,0.956734171124)(560,0.956765867488)(570,0.956828889241)(580,0.956787618686)(590,0.956877507804)(600,0.957326822342)(610,0.959335251458)(620,0.959402694364)(630,0.959500028742)(640,0.956532862186)(650,0.959924700977)(660,0.960548564831)(670,0.960587167906)(680,0.960694013599)(690,0.960725599469)(700,0.961080919371)(710,0.961062574734)(720,0.961060350297)(730,0.961222646705)(740,0.961487113275)(750,0.961487113275)(760,0.961487113275)(770,0.961552811959)(780,0.96223942945)(790,0.962846291199)(800,0.963009183237)(810,0.963009183237)(820,0.963009183237)};
%\addlegendentry{Metadata}


\addplot+[mark=none] coordinates{(4,0.0299178945001)(8,0.0254892821164)(12,0.0335232392871)(16,0.0370730417751)(20,0.0332287993616)(24,0.0343499260897)(28,0.0360758831279)(32,0.0371827706465)(36,0.0378060049643)(40,0.0385790530593)(50,0.0372729271895)(60,0.0404868860914)(70,0.0394720690183)(80,0.0370837384462)(90,0.0407442721244)(100,0.0403147316723)(110,0.0390750929496)(120,0.0334037470965)(130,0.0169159824542)(140,0.0)(150,0.143009238813)(160,0.201278307352)(170,0.244759279505)(180,0.287940620214)(190,0.331272588311)(200,0.349310834551)(210,0.373927956629)(220,0.409433325776)(230,0.425529243178)(240,0.455286918314)(250,0.49688482923)(260,0.557884736267)(270,0.609724108634)(280,0.632880681289)(290,0.647445593335)(300,0.638973769068)(310,0.67608903766)(320,0.668158109641)(330,0.696932960376)(340,0.712527126448)(350,0.713553829986)(360,0.72266833615)(370,0.738739598868)(380,0.75404949824)(390,0.76990442617)(400,0.763199497504)(410,0.791533078806)(420,0.801880067716)(430,0.823038876104)(440,0.835133360855)(450,0.84190278706)(460,0.85070409592)(470,0.855603830222)(480,0.855483810492)(490,0.869505512715)(500,0.874427885835)(510,0.876990939843)(520,0.893757569612)(530,0.903564698038)(540,0.912791092565)(550,0.917403971778)(560,0.916594363672)(570,0.922801450725)(580,0.925422366161)(590,0.929746684885)(600,0.932612339692)(610,0.934835714184)(620,0.935244079542)(630,0.93669451321)(640,0.937514777422)(650,0.93957494791)(660,0.939273105073)(670,0.941552628504)(680,0.941727241359)(690,0.942967068624)(700,0.942526539002)(710,0.9432306921)(720,0.944179854641)(730,0.945906670303)(740,0.946502417335)(750,0.948182983225)(760,0.948683431692)(770,0.949232675885)(780,0.949944804581)(790,0.950553935255)(800,0.951181855556)(810,0.951667167566)(820,0.951916120585)};
%\addlegendentry{Word unigrams}

\addplot+[mark=none] coordinates{(4,0.0427398492858)(8,0.0254284134881)(12,0.0335431540704)(16,0.0377965937993)(20,0.0327689787002)(24,0.0331144608538)(28,0.0355431985121)(32,0.0373797858828)(36,0.0386114010969)(40,0.039813795573)(50,0.0385525870815)(60,0.042691476551)(70,0.0414795889613)(80,0.0398769660348)(90,0.0453044134093)(100,0.047776955024)(110,0.046892822441)(120,0.0452060684233)(130,0.0422899561354)(140,0.0)(150,0.0838765620699)(160,0.08716906007)(170,0.101145014278)(180,0.131136828115)(190,0.193261236727)(200,0.228595301838)(210,0.287174553115)(220,0.300726574113)(230,0.334213810857)(240,0.350820114383)(250,0.378875296206)(260,0.403188952701)(270,0.433327765531)(280,0.456792711284)(290,0.478132494302)(300,0.498154805985)(310,0.5089949228)(320,0.539099209041)(330,0.577787789768)(340,0.598743317003)(350,0.605283676046)(360,0.619564050094)(370,0.63469454322)(380,0.632471331952)(390,0.657876679218)(400,0.678348901642)(410,0.686762317976)(420,0.706189777202)(430,0.710903245485)(440,0.716090670114)(450,0.725987508451)(460,0.739073799814)(470,0.747726956259)(480,0.749506033868)(490,0.756066614767)(500,0.768261994841)(510,0.780139103048)(520,0.787724441746)(530,0.790287122171)(540,0.801615125656)(550,0.80330187684)(560,0.813574243577)(570,0.812080803702)(580,0.812813591569)(590,0.819466403898)(600,0.831232843492)(610,0.842502107135)(620,0.846682047464)(630,0.854564521152)(640,0.862229739817)(650,0.86752394011)(660,0.868954963473)(670,0.874644078019)(680,0.879766687018)(690,0.884421481707)(700,0.889857782986)(710,0.889628184782)(720,0.898040394602)(730,0.905705845272)(740,0.908884329692)(750,0.909601658457)(760,0.91121744046)(770,0.912114424857)(780,0.914357630378)(790,0.91491458856)(800,0.920761025151)(810,0.922385357587)(820,0.924313589784)};
%\addlegendentry{Word2Vec}


\addplot+[mark=none] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(20,0.0)(24,0.0)(28,0.0)(32,0.0)(36,0.0)(40,0.0)(50,0.00495622783688)(60,0.00495622783688)(70,0.00732620808704)(80,0.0090533416348)(90,0.00944963584827)(100,0.00984435746566)(110,0.0115489933994)(120,0.0119458139005)(130,0.0128638046202)(140,0.0149693801925)(150,0.153720928564)(160,0.320345390722)(170,0.402057671131)(180,0.448401252328)(190,0.523055821594)(200,0.561661111603)(210,0.566069429748)(220,0.583732255868)(230,0.602569657597)(240,0.604969981038)(250,0.641679932562)(260,0.656237791027)(270,0.716104137586)(280,0.733510623608)(290,0.772136295289)(300,0.787409707193)(310,0.8292621786)(320,0.839776769089)(330,0.863592459543)(340,0.871721623772)(350,0.897531129055)(360,0.925375692229)(370,0.933576367527)(380,0.933787829811)(390,0.934174301877)(400,0.940364512784)(410,0.940069721577)(420,0.940472386741)(430,0.944600635794)(440,0.948592976117)(450,0.949078894384)(460,0.951017630976)(470,0.951102977193)(480,0.951537533693)(490,0.951837624057)(500,0.952037081222)(510,0.952480921409)(520,0.953690670023)(530,0.954762041802)(540,0.955779132088)(550,0.95638356551)(560,0.95676631808)(570,0.957342526865)(580,0.957947010593)(590,0.957991728743)(600,0.958918071179)(610,0.957436744883)(620,0.959426633463)(630,0.960359566798)(640,0.961837151608)(650,0.961967741677)(660,0.962005279814)(670,0.962655203223)(680,0.962917744697)(690,0.96437588925)(700,0.964165645901)(710,0.964769784329)(720,0.966048659924)(730,0.967322884217)(740,0.967733052641)(750,0.968814746552)(760,0.969724042044)(770,0.970148062773)(780,0.970310025463)(790,0.970457096124)(800,0.971063899019)(810,0.971063899019)(820,0.971129279749)};
%\addlegendentry{Char unigrams + Metadata + Word2Vec}

\addplot+[mark=none] coordinates{(4,0.0341918794286)(8,0.0276497142874)(12,0.0318037195359)(16,0.0329111969282)(20,0.0276330065822)(24,0.0282642184562)(28,0.0352771308471)(32,0.0369852545497)(36,0.0380800969031)(40,0.0391433604189)(50,0.0370306581367)(60,0.0405408008074)(70,0.0397241374339)(80,0.0373830823835)(90,0.0406254459191)(100,0.0418030736262)(110,0.0402158737002)(120,0.0341669268143)(130,0.0211449780677)(140,0.0)(150,0.0912632170429)(160,0.123937238749)(170,0.203627773916)(180,0.273319805706)(190,0.335073039134)(200,0.350746526699)(210,0.423147890656)(220,0.475329196743)(230,0.498856629035)(240,0.572537603181)(250,0.637588760445)(260,0.654677560418)(270,0.696872674316)(280,0.734466410621)(290,0.767975578839)(300,0.792723146875)(310,0.808363943469)(320,0.8347592077)(330,0.871064158369)(340,0.902938361189)(350,0.921862078151)(360,0.930638604841)(370,0.93182443004)(380,0.943702776533)(390,0.945500669729)(400,0.947596414011)(410,0.948210651338)(420,0.946636486754)(430,0.950435521875)(440,0.951073420619)(450,0.947711252143)(460,0.933222474576)(470,0.944734997518)(480,0.94700377147)(490,0.950355577115)(500,0.953020632773)(510,0.953460809754)(520,0.955510079625)(530,0.955298521578)(540,0.955172832876)(550,0.943622567879)(560,0.956800951992)(570,0.957395595852)(580,0.957388737061)(590,0.958070670133)(600,0.957935481554)(610,0.959665708758)(620,0.959994834957)(630,0.961341492132)(640,0.961829388736)(650,0.962171525355)(660,0.962401708222)(670,0.963065624119)(680,0.96316304128)(690,0.963400647307)(700,0.963308072932)(710,0.966175894307)(720,0.966275690368)(730,0.966892471759)(740,0.966985796594)(750,0.96707361628)(760,0.967073830574)(770,0.967944601451)(780,0.967978375188)(790,0.968299952506)(800,0.969014651095)(810,0.969848054659)(820,0.970249875377)};
%\addlegendentry{Char unigrams + Metadata + Error correlation + Word2Vec}





==> charts/labels_all/labels_address.tex <==

\nextgroupplot[legend to name=testLegendlabels,
title={Address},
%ylabel={$F_1$-score},
xmax=\limitaddress]

%/home/neutatz/logs/out/features/labels_experiment_data_BlackOakUppercase_char unigrams + meta data + correlation + word2vec_time_1536953982.69.csv

%boxplotlabels{label}{median}{lower_quartile}{upper_quartile}{minimum}{maximum}                

\iffalse
\boxplotlabels{4}{0.0}{0.0}{0.000111408642923}{0.0}{0.000111408642923}
\boxplotlabels{8}{0.000111408642923}{0.0}{0.000809027569329}{0.0}{0.00132098819466}
\boxplotlabels{12}{0.000576487927194}{0.0}{0.00327701428443}{0.0}{0.00480856862626}
\boxplotlabels{16}{0.0868103651202}{2.78521607308e-05}{0.172478457241}{0.0}{0.295606918477}
\boxplotlabels{20}{0.170825955417}{2.78521607308e-05}{0.242570965442}{0.0}{0.531089334641}
\boxplotlabels{24}{0.324445841473}{0.262152139003}{0.341138227114}{0.000111408642923}{0.60259263216}
\boxplotlabels{28}{0.347149839953}{0.294553996762}{0.372620669901}{0.000111408642923}{0.584660595794}
\boxplotlabels{38}{0.364322244477}{0.332645626528}{0.372620669901}{0.0}{0.584660595794}
\boxplotlabels{48}{0.365705660212}{0.332645626528}{0.419044974586}{0.0}{0.584660595794}
\boxplotlabels{58}{0.411745984903}{0.33648954858}{0.459423583087}{0.0}{0.584660595794}
\boxplotlabels{68}{0.385676884507}{0.334643808896}{0.445272007887}{0.0229043003481}{0.552744298812}
\boxplotlabels{78}{0.595156786381}{0.54346772985}{0.605505738986}{0.503175394628}{0.615741075478}
\boxplotlabels{88}{0.539860529882}{0.537221880754}{0.543094416964}{0.509184444025}{0.614874984582}
\boxplotlabels{98}{0.68921653653}{0.68191779436}{0.697664270042}{0.654361241284}{0.744641334067}
\boxplotlabels{108}{0.706967912694}{0.686397524749}{0.737496774655}{0.658731911135}{0.865789994423}
\boxplotlabels{118}{0.848193582776}{0.84601013142}{0.854588715971}{0.82997004484}{0.952244353502}
\boxplotlabels{128}{0.965541301071}{0.891207975246}{0.971553909297}{0.848281728978}{0.975228365541}
\boxplotlabels{138}{0.974640938674}{0.957920360059}{0.975441557225}{0.896435246155}{0.98405842348}
\boxplotlabels{148}{0.972800263591}{0.97207123387}{0.97479564308}{0.962639321193}{0.990690906765}
\boxplotlabels{158}{0.975515551053}{0.972189153733}{0.976369059485}{0.962639321193}{0.990690906765}
\boxplotlabels{168}{0.976209124679}{0.973430862323}{0.976471488386}{0.957574095452}{0.990690906765}
\boxplotlabels{178}{0.976209124679}{0.972236776609}{0.976471488386}{0.962848069016}{0.990690906765}
\boxplotlabels{188}{0.97644381353}{0.97631084749}{0.976611599287}{0.962848069016}{0.990700589688}
\boxplotlabels{198}{0.976361318506}{0.975397521979}{0.976611599287}{0.941601489507}{0.984981105884}
\boxplotlabels{208}{0.976770265192}{0.959135780579}{0.98653915528}{0.939123466808}{0.991552381959}
\boxplotlabels{218}{0.979585110128}{0.971956213896}{0.985941487109}{0.961173502422}{0.990842127493}
\boxplotlabels{228}{0.981694284528}{0.974914558014}{0.986804462008}{0.964072213688}{0.990842127493}
\boxplotlabels{238}{0.98557504341}{0.977692575642}{0.986578596174}{0.963018637097}{0.990961532924}
\boxplotlabels{248}{0.986752604591}{0.98569695585}{0.987053381643}{0.983607398641}{0.991826852249}
\boxplotlabels{258}{0.986866471814}{0.986228786892}{0.987190321569}{0.985279502906}{0.990721629721}
\boxplotlabels{268}{0.986749019233}{0.986102182719}{0.987181352271}{0.985578471408}{0.991427757159}
\boxplotlabels{278}{0.986944543473}{0.986228786892}{0.987611466634}{0.985578471408}{0.992074344252}
\boxplotlabels{288}{0.987185265102}{0.986267926196}{0.989852175685}{0.985578471408}{0.992150696382}
\boxplotlabels{298}{0.987244352518}{0.986893911233}{0.989852175685}{0.985656917057}{0.992150696382}
\boxplotlabels{308}{0.987245983984}{0.986365731116}{0.989893359617}{0.968755389947}{0.992150696382}
\boxplotlabels{318}{0.987323332986}{0.986387087364}{0.987543442326}{0.985361862239}{0.992135011368}
\boxplotlabels{328}{0.987355005087}{0.986387087364}{0.98993784651}{0.985361862239}{0.992135263225}
\boxplotlabels{338}{0.987358267988}{0.986388718505}{0.989991940062}{0.985443945177}{0.992049998879}
\boxplotlabels{348}{0.987557222901}{0.987293857742}{0.990243675094}{0.985986613791}{0.992049998879}
\boxplotlabels{358}{0.987557222901}{0.987176077597}{0.99065353467}{0.985986613791}{0.992068904792}
\boxplotlabels{368}{0.987557222901}{0.987283547543}{0.99203310935}{0.985993136476}{0.99247518668}
\boxplotlabels{378}{0.987425154526}{0.986526701488}{0.990938446354}{0.984649484929}{0.99247518668}
\boxplotlabels{388}{0.987425154526}{0.986784276526}{0.990860787761}{0.9847808274}{0.99247518668}
\boxplotlabels{398}{0.987571158545}{0.986792378589}{0.99091111244}{0.9847808274}{0.992562105142}
\boxplotlabels{408}{0.98771728341}{0.98719654692}{0.991019856731}{0.9847808274}{0.992562105142}
\boxplotlabels{418}{0.988342759436}{0.987312905787}{0.992007770816}{0.984776216093}{0.992584674567}
\boxplotlabels{428}{0.988342759436}{0.987312905787}{0.992288068041}{0.984940964261}{0.992584674567}
\boxplotlabels{438}{0.988342759436}{0.986920138716}{0.992233772488}{0.982704412667}{0.992739780818}
\boxplotlabels{448}{0.988384199115}{0.987624074849}{0.992391379982}{0.985316481416}{0.992765425067}
\boxplotlabels{458}{0.991682818149}{0.987991948952}{0.992471781703}{0.985316294944}{0.992765425067}
\boxplotlabels{468}{0.991981302627}{0.988100290712}{0.992471781703}{0.985344635997}{0.992765425067}
\boxplotlabels{478}{0.99198452328}{0.988060798151}{0.992486406126}{0.985344635997}{0.992787015348}
\boxplotlabels{488}{0.992302871826}{0.989670837973}{0.992503617401}{0.986233313838}{0.992812247981}
\boxplotlabels{498}{0.992359771154}{0.989707907116}{0.992509467188}{0.986233313838}{0.992811971939}
\boxplotlabels{508}{0.992360315704}{0.989707907116}{0.992670056108}{0.986922047163}{0.992828088546}
\boxplotlabels{518}{0.992380837433}{0.989707907116}{0.99267485849}{0.987915505109}{0.992853370885}
\boxplotlabels{528}{0.992382401021}{0.989707907116}{0.992680514727}{0.987915505109}{0.992888462154}
\boxplotlabels{538}{0.992646654111}{0.992317617461}{0.992862855885}{0.987915505109}{0.99309479774}
\boxplotlabels{548}{0.992569199782}{0.992299082096}{0.992755322724}{0.988132521783}{0.99309479774}
\boxplotlabels{558}{0.992679367914}{0.992322485682}{0.992871649181}{0.988132521783}{0.99309479774}
\boxplotlabels{568}{0.992704619022}{0.992370402132}{0.992898452807}{0.988132521783}{0.993902497514}
\fi

\addplot+[mark=triangle*] coordinates{(4,4.45634571693e-05)(8,0.000401776952956)(12,0.00151405786374)(16,0.102986156585)(20,0.168692369467)(24,0.299310549265)(28,0.316450328544)(38,0.333690249254)(48,0.356212861314)(58,0.383992415879)(68,0.351390870142)(78,0.575584076576)(88,0.544763180182)(98,0.693109364852)(108,0.729302411522)(118,0.858050140293)(128,0.93598471838)(138,0.962349333092)(148,0.973146984141)(158,0.974129484454)(168,0.97499788574)(178,0.97491784508)(188,0.976404404999)(198,0.972343688948)(208,0.971456016017)(218,0.977834301847)(228,0.979871635811)(238,0.981756209138)(248,0.986703610732)(258,0.986976167439)(268,0.987344943384)(278,0.987564802939)(288,0.987944209127)(298,0.988111764875)(308,0.986316693024)(318,0.987716197123)(328,0.988055577082)(338,0.988107418055)(348,0.988451962113)(358,0.988653211595)(368,0.989055855826)(378,0.988326913539)(388,0.988418249848)(398,0.988479513195)(408,0.988624982513)(418,0.989166906776)(428,0.989280488234)(438,0.988873299689)(448,0.989466146707)(458,0.990322222753)(468,0.990398402971)(478,0.99027220788)(488,0.990996389836)(498,0.991029574612)(508,0.991137802295)(518,0.991248242689)(528,0.99125465281)(538,0.991851375654)(548,0.991827958468)(558,0.991890926059)(568,0.992003594533)};
%\addlegendimage{mark=square,black}
\addlegendentry{\system{}}

%/home/neutatz/logs/out/features/labels_experiment_data_BlackOakUppercase_ActiveClean_time_1536888775.32.csv
\addplot+ coordinates{(4,4.45634571693e-05)(8,0.00026967813349)(12,0.00296953220593)(16,0.0794803426546)(20,0.309227331935)(24,0.331781115174)(28,0.341940789739)(38,0.373937776528)(48,0.38318503373)(58,0.431604366634)(68,0.377022117362)(78,0.463594307262)(88,0.447178051749)(98,0.457693716468)(108,0.444169185321)(118,0.433841431723)(128,0.436027856801)(138,0.446997664773)(148,0.444133519999)(158,0.451440639278)(168,0.453464519443)(178,0.462634532095)(188,0.458050026135)(198,0.459015462205)(208,0.466972286665)(218,0.466033864053)(228,0.470326424972)(238,0.475008892487)(248,0.475582227657)(258,0.478319669306)(268,0.482236998148)(278,0.481210105211)(288,0.482732243747)(298,0.483739734737)(308,0.482965222631)(318,0.482826110127)(328,0.481833295371)(338,0.482714043861)(348,0.483450459767)(358,0.483057273082)(368,0.481390861907)(378,0.482994745747)(388,0.483225274193)(398,0.48480137212)(408,0.486022886742)(418,0.487025161338)(428,0.490507879918)(438,0.490749361468)(448,0.492805502637)(458,0.493591902821)(468,0.496470446858)(478,0.49616612598)(488,0.497252307307)(498,0.496385871928)(508,0.496414428405)(518,0.49681014915)(528,0.497318323861)(538,0.499322242952)(548,0.501399888177)(558,0.502178845039)(568,0.502235808268)};
\addlegendentry{ActiveClean}

\addplot+ coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(20,0.0)(24,0.0)(28,0.0)(38,0.0)(48,0.0)(58,0.0)(68,0.0129589691005)(78,0.301586110503)(88,0.310434129785)(98,0.358605419942)(108,0.366190970298)(118,0.380615995017)(128,0.417497012036)(138,0.450449179407)(148,0.500186227953)(158,0.535794613128)(168,0.559752847316)(178,0.589787399207)(188,0.58625570399)(198,0.591593365326)(208,0.632210390806)(218,0.637395096046)(228,0.658018227258)(238,0.652780828608)(248,0.656430946895)(258,0.644107648053)(268,0.657092657115)(278,0.660947917804)(288,0.650827628165)(298,0.659761825838)(308,0.659351986415)(318,0.655687837351)(328,0.662046352017)(338,0.690670707942)(348,0.680048274066)(358,0.678669479844)(368,0.695111650775)(378,0.693623593565)(388,0.692719139702)(398,0.695501052778)(408,0.704229773906)(418,0.687136407308)(428,0.687359687596)(438,0.701144221954)(448,0.687637376335)(458,0.698970880717)(468,0.713918904593)(478,0.719394030223)(488,0.721449752745)(498,0.7176606841)(508,0.71095327668)(518,0.717178758976)(528,0.727096866423)(538,0.719738418804)(548,0.726655142114)(558,0.733079372313)(568,0.721195609132)};
\addlegendentry{BoostClean}


%\addplot+[no marks] coordinates{(0,0.904)(201,0.904)};
%\addlegendentry{OpenRefine}

\addplot+[no marks, line width=2] coordinates{(0,0.26)(201,0.26)};
\addlegendentry{KATARA}

\addplot+[no marks, line width=2] coordinates{(0,0.904277255311738)(201,0.904277255311738)};
\addlegendentry{NADEEF}

%\addplot+[mark=x] coordinates{(0,0.2986000962729733)(201,0.2986000962729733)};%check
%\addlegendentry{Gaussian}

%\addplot+[mark=x] coordinates{(0,0.257099700907)(201,0.257099700907)};
%\addlegendentry{Histogram}

\addplot+[mark=x] coordinates{(0,0.4547430518594286)(201,0.4547430518594286)};
\addlegendentry{dBoost}


\addplot coordinates{(0,0.0)(0,0.00)(10,0.70)(20,0.73)(30,0.86)(40,0.83)(50,0.88)(60,0.87)(70,0.89)(80,0.88)(90,0.88)(100,0.90)(110,0.90)(120,0.90)(130,0.90)(140,0.90)(150,0.90)};
\addlegendentry{MDED}






==> charts/labels_all/labels_beers.tex <==
\nextgroupplot[title={Beers},
%ylabel={$F_1$-score},
xmax=\limitbeers]


%/home/neutatz/logs/out/features_beers/labels_experiment_data_Beers_char unigrams + meta data + correlation + word2vec_XGBoost_time_1537448053.36.csv
                
%addplot
%boxplotlabels{label}{median}{lower_quartile}{upper_quartile}{minimum}{maximum}
\iffalse
\boxplotlabels{4}{0.0}{0.0}{0.0}{0.0}{0.0}
\boxplotlabels{8}{0.0}{0.0}{0.0}{0.0}{0.0}
\boxplotlabels{12}{0.0}{0.0}{0.0}{0.0}{0.0}
\boxplotlabels{16}{0.0}{0.0}{0.0}{0.0}{0.0}
\boxplotlabels{26}{0.419994120987}{0.0347067833531}{0.52371947266}{0.0}{0.524007561437}
\boxplotlabels{36}{0.425314413243}{0.0465744211191}{0.526186670655}{0.00510986203373}{0.530673692134}
\boxplotlabels{46}{0.425911955975}{0.0480502916164}{0.526186670655}{0.0101936799185}{0.530673692134}
\boxplotlabels{56}{0.427350457489}{0.0516493069264}{0.527020561839}{0.0132315521628}{0.530673692134}
\boxplotlabels{66}{0.606436041323}{0.528863372204}{0.747931448043}{0.290718038529}{0.89592760181}
\boxplotlabels{76}{0.823175924908}{0.693753351981}{0.930410958904}{0.549777117385}{0.931874145007}
\boxplotlabels{86}{0.930703836517}{0.930410958904}{0.931947064282}{0.73534175575}{0.949407965554}
\boxplotlabels{96}{0.931581508049}{0.930410958904}{0.940578357327}{0.74791533034}{0.967195767196}
\boxplotlabels{106}{0.941140745274}{0.931508588906}{0.96299327866}{0.74791533034}{0.984927234927}
\boxplotlabels{116}{0.949517345557}{0.934123368888}{0.973577833322}{0.931289351218}{0.984927234927}
\boxplotlabels{126}{0.949517345557}{0.934123368888}{0.973577833322}{0.931289351218}{0.984927234927}
\boxplotlabels{136}{0.962379799046}{0.934123368888}{0.981920893178}{0.931874145007}{0.998460749102}
\boxplotlabels{146}{0.97513213731}{0.938162159632}{0.990366574264}{0.931874145007}{0.998974358974}
\boxplotlabels{156}{0.986488975575}{0.967195767196}{0.990366574264}{0.931911402789}{1.0}
\boxplotlabels{166}{0.986488975575}{0.968219237535}{0.990366574264}{0.967758985201}{1.0}
\boxplotlabels{176}{0.986488975575}{0.968219237535}{0.990366574264}{0.967758985201}{1.0}
\boxplotlabels{186}{0.986753732537}{0.972391532561}{0.990366574264}{0.968014803066}{1.0}
\boxplotlabels{196}{0.986884370219}{0.972391532561}{0.996838734061}{0.968014803066}{1.0}
\boxplotlabels{206}{0.995476867408}{0.985306480842}{1.0}{0.968014803066}{1.0}
\boxplotlabels{216}{0.995476867408}{0.985306480842}{1.0}{0.968014803066}{1.0}
\boxplotlabels{226}{1.0}{0.985436949715}{1.0}{0.968014803066}{1.0}
\boxplotlabels{236}{1.0}{0.992701954089}{1.0}{0.971819857782}{1.0}
\boxplotlabels{246}{1.0}{0.992701954089}{1.0}{0.971819857782}{1.0}
\boxplotlabels{256}{1.0}{0.992701954089}{1.0}{0.971819857782}{1.0}
\boxplotlabels{266}{1.0}{1.0}{1.0}{0.990953734815}{1.0}
\boxplotlabels{276}{1.0}{1.0}{1.0}{1.0}{1.0}
\boxplotlabels{286}{1.0}{1.0}{1.0}{1.0}{1.0}
\boxplotlabels{296}{1.0}{1.0}{1.0}{1.0}{1.0}
\boxplotlabels{306}{1.0}{1.0}{1.0}{1.0}{1.0}
\boxplotlabels{316}{1.0}{1.0}{1.0}{1.0}{1.0}
\boxplotlabels{326}{1.0}{1.0}{1.0}{1.0}{1.0}
\boxplotlabels{336}{1.0}{1.0}{1.0}{1.0}{1.0}
\boxplotlabels{346}{1.0}{1.0}{1.0}{1.0}{1.0}
\boxplotlabels{356}{1.0}{1.0}{1.0}{1.0}{1.0}
\boxplotlabels{366}{1.0}{1.0}{1.0}{1.0}{1.0}
\boxplotlabels{376}{1.0}{1.0}{1.0}{1.0}{1.0}
\boxplotlabels{386}{1.0}{1.0}{1.0}{1.0}{1.0}
\boxplotlabels{396}{1.0}{1.0}{1.0}{1.0}{1.0}
\boxplotlabels{406}{1.0}{1.0}{1.0}{1.0}{1.0}
\boxplotlabels{416}{1.0}{1.0}{1.0}{1.0}{1.0}
\boxplotlabels{426}{1.0}{1.0}{1.0}{1.0}{1.0}
\boxplotlabels{436}{1.0}{1.0}{1.0}{1.0}{1.0}
\boxplotlabels{446}{1.0}{1.0}{1.0}{1.0}{1.0}
\fi

\addplot+[mark=triangle*] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(26,0.303471271536)(36,0.309141949558)(46,0.31027040985)(56,0.312126678446)(66,0.633352726288)(76,0.80106420655)(86,0.894527437519)(96,0.919492627368)(106,0.929737666913)(116,0.954705911143)(126,0.954705911143)(136,0.960716658855)(146,0.968040354349)(156,0.975102412769)(166,0.982517602081)(176,0.982517602081)(186,0.984101505696)(196,0.985110561323)(206,0.990481827634)(216,0.990481827634)(226,0.991438641701)(236,0.994431822586)(246,0.994431822586)(256,0.994431822586)(266,0.998890034672)(276,1.0)(286,1.0)(296,1.0)(306,1.0)(316,1.0)(326,1.0)(336,1.0)(346,1.0)(356,1.0)(366,1.0)(376,1.0)(386,1.0)(396,1.0)(406,1.0)(416,1.0)(426,1.0)(436,1.0)(446,1.0)};
%\addlegendimage{mark=square,black}
%\addlegendentry{ED2}

\addplot+ coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(26,0.160959275634)(36,0.1949604208)(46,0.190504076118)(56,0.190872657712)(66,0.18932661202)(76,0.192149195039)(86,0.196069003708)(96,0.198886583497)(106,0.205343354034)(116,0.207655302615)(126,0.224703135305)(136,0.194181266513)(146,0.188280411231)(156,0.181626968953)(166,0.172028417331)(176,0.168088897228)(186,0.165281782792)(196,0.16641112019)(206,0.155788598629)(216,0.147605683355)(226,0.140291838607)(236,0.135809417343)(246,0.130457203815)(256,0.130491930209)(266,0.131079354508)(276,0.125649927283)(286,0.123794746955)(296,0.121651741176)(306,0.120631392118)(316,0.121019155458)(326,0.12038741056)(336,0.119369442751)(346,0.118755018163)(356,0.119782837772)(366,0.11863117108)(376,0.119830608069)(386,0.121804342146)(396,0.123245144059)(406,0.122626172259)(416,0.123625960161)(426,0.1249724257)(436,0.124816786419)(446,0.124718605096)};
%\addlegendentry{ActiveClean Features}

\addplot+ coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(26,0.0618506341639)(36,0.0687748221401)(46,0.0730031203278)(56,0.074114190429)(66,0.0955942287983)(76,0.311309554507)(86,0.578595595064)(96,0.693639459256)(106,0.689711264728)(116,0.68235517655)(126,0.639418509914)(136,0.688251391968)(146,0.612618018137)(156,0.663819697277)(166,0.675108225245)(176,0.685103507898)(186,0.666750425359)(196,0.670831805958)(206,0.670970464255)(216,0.671812173509)(226,0.667013333758)(236,0.682796773339)(246,0.668242203382)(256,0.665087789345)(266,0.653153834916)(276,0.681821335382)(286,0.651027475956)(296,0.683818487131)(306,0.678222274494)(316,0.675426584568)(326,0.674555452413)(336,0.698493835377)(346,0.680471745424)(356,0.67442559835)(366,0.656635792665)(376,0.660034202405)(386,0.691879956896)(396,0.690763884562)(406,0.691568305841)(416,0.689079960525)(426,0.691124623688)(436,0.67389137514)(446,0.69045944359)};
%\addlegendentry{BoostClean Features}


\addplot+[no marks, line width=2] coordinates{(0,0.21)(801,0.21)}; 
%\addlegendentry{KATARA}

\addplot+[no marks, line width=5] coordinates{(0, 1.00)(801, 1.00)}; %done
%\addlegendentry{NADEEF}



%\addplot+[mark=x] coordinates{(0,0.37)(801,0.37)}; %0.24778917580474, 0.7177254098360656, 0.3683933736523797
%\addlegendentry{Gaussian}
\addplot+[mark=x] coordinates{(0,0.57)(801,0.57)}; %0.3965867533522958, 1.0, 0.5679371544951993
%\addlegendentry{Histogram}
%\addplot+[mark=x] coordinates{(0,0.23)(801,0.23)}; %0.9477611940298507, 0.13012295081967212, 0.22882882882882882
%\addlegendentry{Mixture}

\addplot coordinates{(0,0.0)(0,0.00)(10,0.70)(20,1.00)(30,1.00)(40,1.00)(50,1.00)(60,1.00)(70,1.00)(80,1.00)(90,1.00)(100,1.00)(110,1.00)(120,1.00)(130,1.00)(140,1.00)(150,1.00)(160,1.00)(170,1.00)(180,1.00)(190,1.00)(200,1.00)(210,1.00)(220,1.00)(230,1.00)(240,1.00)(250,1.00)(260,1.00)(270,1.00)(280,1.00)(290,1.00)(300,1.00)(310,1.00)(320,1.00)(330,1.00)(340,1.00)}; %\addlegendentry{Metadata Driven}








==> charts/labels_all/labels_flights.tex <==
\nextgroupplot[title={Flights},
ylabel={$F_1$-score}, xmax=\limitflights]

%/home/neutatz/logs/out/features/labels_experiment_data_Flight HoloClean_char unigrams + meta data + correlation + word2vec_time_1536953982.68.csv
                
%addplot
%boxplotlabels{label}{median}{lower_quartile}{upper_quartile}{minimum}{maximum}
\iffalse
\boxplotlabels{4}{0.249725877193}{0.0}{0.249725877193}{0.0}{0.249725877193}
\boxplotlabels{8}{0.427083333333}{0.294065241228}{0.489680262614}{0.249725877193}{0.510545905707}
\boxplotlabels{12}{0.530086848635}{0.294065241228}{0.549627791563}{0.249725877193}{0.592463479416}
\boxplotlabels{16}{0.571045635489}{0.437247983871}{0.657661022576}{0.249725877193}{0.682196339434}
\boxplotlabels{26}{0.670079588137}{0.557782915063}{0.746302694035}{0.301398239254}{0.756054158607}
\boxplotlabels{36}{0.681658946837}{0.603383457828}{0.739045020958}{0.561054330285}{0.765062213491}
\boxplotlabels{46}{0.757350580688}{0.640291293222}{0.791828869722}{0.605783518116}{0.813402245589}
\boxplotlabels{56}{0.808291907255}{0.768526898707}{0.835851148633}{0.743176776931}{0.850736214031}
\boxplotlabels{66}{0.82146819281}{0.775037302005}{0.835098779019}{0.733943089431}{0.848193225776}
\boxplotlabels{76}{0.832753313788}{0.789843833095}{0.837795979926}{0.746455131383}{0.874432969791}
\boxplotlabels{86}{0.833769038418}{0.81555446892}{0.845766970894}{0.763738390093}{0.855143031041}
\boxplotlabels{96}{0.850376772157}{0.836840285845}{0.866012157774}{0.802781041911}{0.875815738964}
\boxplotlabels{106}{0.866748437419}{0.858981179873}{0.871667285838}{0.834838709677}{0.875827020807}
\boxplotlabels{116}{0.868615836663}{0.863315545082}{0.875657884417}{0.843819806404}{0.889864325619}
\boxplotlabels{126}{0.876680948357}{0.87587483872}{0.881592304239}{0.849299289691}{0.895672791938}
\boxplotlabels{136}{0.884301022167}{0.874964344866}{0.895700285217}{0.863801750418}{0.899872761084}
\boxplotlabels{146}{0.896120586064}{0.884537261446}{0.903257160947}{0.874259636858}{0.915902910666}
\boxplotlabels{156}{0.89989291797}{0.890804041967}{0.912828317517}{0.873608903021}{0.921639541893}
\boxplotlabels{166}{0.905234065804}{0.89535836713}{0.921278130797}{0.889652384802}{0.928046694173}
\boxplotlabels{176}{0.913240318488}{0.907770407267}{0.924365324085}{0.895610913405}{0.928808780586}
\boxplotlabels{186}{0.915750562448}{0.911343238455}{0.926897970767}{0.905093728531}{0.933613277345}
\boxplotlabels{196}{0.923951139632}{0.91953474601}{0.930640026665}{0.918433770589}{0.9364}
\boxplotlabels{206}{0.931046083898}{0.92860595862}{0.934426634677}{0.920539730135}{0.936303164685}
\boxplotlabels{216}{0.936307468122}{0.93516161285}{0.938770521632}{0.926926527764}{0.942163620018}
\boxplotlabels{226}{0.934939522239}{0.933093268252}{0.939883818522}{0.932111959288}{0.946312092323}
\boxplotlabels{236}{0.939771918449}{0.935148666595}{0.942297578557}{0.93458890239}{0.950568811034}
\boxplotlabels{246}{0.945464838604}{0.937193892655}{0.94733946005}{0.934635914996}{0.951432880845}
\boxplotlabels{256}{0.946231225066}{0.94172233634}{0.948774320849}{0.93683148335}{0.954992967651}
\boxplotlabels{266}{0.949044811428}{0.945735525817}{0.952869570365}{0.94178939986}{0.956835976712}
\boxplotlabels{276}{0.953808658795}{0.948379652854}{0.955577223337}{0.94510355922}{0.956853301224}
\boxplotlabels{286}{0.955865714697}{0.952121459064}{0.956451686169}{0.94948464129}{0.957653418761}
\fi


\addplot+[mark=triangle*] coordinates{(4,0.149835526316)(8,0.398914868203)(12,0.452061720414)(16,0.518370407585)(26,0.606981642212)(36,0.673061242558)(46,0.723728159379)(56,0.802557955001)(66,0.807788557533)(76,0.818339593458)(86,0.823993108043)(96,0.846648110953)(106,0.863539600343)(116,0.868669437322)(126,0.877020227908)(136,0.883791043541)(146,0.894611663651)(156,0.901100040873)(166,0.90762223086)(176,0.913568866176)(186,0.918054828067)(196,0.925218115668)(206,0.930948529106)(216,0.936005853192)(226,0.936924621927)(236,0.939750771895)(246,0.9432631608)(256,0.945926393)(266,0.949207576361)(276,0.952194338124)(286,0.954405069363)};
%\addlegendimage{mark=square,black}
%\addlegendentry{ED2}

\addplot+ coordinates{(4,0.174808114035)(8,0.338470789256)(12,0.447096356477)(16,0.51740921844)(26,0.471758066451)(36,0.461091526226)(46,0.412857759601)(56,0.449235943334)(66,0.495306740556)(76,0.493583329858)(86,0.515994109141)(96,0.53024253579)(106,0.519066108727)(116,0.541041580464)(126,0.543805915464)(136,0.546086191858)(146,0.556148743783)(156,0.570206226721)(166,0.587610503729)(176,0.596920575295)(186,0.60061029651)(196,0.603225987233)(206,0.607908764918)(216,0.608652030624)(226,0.612472473831)(236,0.621796420959)(246,0.623875529614)(256,0.626271652383)(266,0.625133966133)(276,0.631287519927)(286,0.634712982939)};
%\addlegendentry{ActiveClean Features}

\addplot+ coordinates{(4,0.249725877193)(8,0.510545905707)(12,0.592463479416)(16,0.682196339434)(26,0.739839061763)(36,0.732921025584)(46,0.75380581144)(56,0.759182521513)(66,0.772964640575)(76,0.782021829829)(86,0.792377560847)(96,0.804265515646)(106,0.821477892185)(116,0.838165878228)(126,0.851520457311)(136,0.862945512051)(146,0.870158851882)(156,0.878226805239)(166,0.885439481084)(176,0.892689653925)(186,0.899407654221)(196,0.906525680146)(206,0.908411993846)(216,0.916923058576)(226,0.921282903748)(236,0.925783861657)(246,0.929230707678)(256,0.93286310554)(266,0.936386766004)(276,0.939279163466)(286,0.9428816986)};
%\addlegendentry{BoostClean Features}


%\addplot+[no marks] coordinates{(0,0.7366)(201,0.7366)};
%\addlegendentry{OpenRefine}


\addplot+[no marks, line width=2] coordinates{(0,0.09)(201,0.09)};
%\addlegendentry{KATARA}

\addplot+[no marks, line width=2] coordinates{(0,0.736)(201,0.736)};
%\addlegendentry{NADEEF}



%\addplot+[mark=x] coordinates{(0,0.538528896673)(201,0.538528896673)};
%\addlegendentry{Gaussian}
%\addplot+[mark=x] coordinates{(0,0.593559042114)(201,0.593559042114)};
%\addlegendentry{Histogram}
\addplot+[mark=x] coordinates{(0,0.6821963394342762)(201,0.6821963394342762)};
%\addlegendentry{Mixture}

\addplot coordinates{(0,0.0)(0,0.00)(10,0.60)(20,0.67)(30,0.71)(40,0.73)(50,0.73)(60,0.74)(70,0.73)(80,0.76)(90,0.77)(100,0.75)(110,0.76)(120,0.77)};
%\addlegendentry{Metadata-driven Error Detection}






==> charts/labels_all/labels_movies.tex <==
\nextgroupplot[title={Movies},
xmax=\limitmovies]

%/home/neutatz/logs/out/features/labels_experiment_data_Movies_char unigrams + meta data + correlation + word2vec_time_1536953982.7.csv
                
%addplot
%boxplotlabels{label}{median}{lower_quartile}{upper_quartile}{minimum}{maximum}
\iffalse
\boxplotlabels{4}{0.0}{0.0}{0.0320548869643}{0.0}{0.0427398492858}
\boxplotlabels{8}{0.0038240917782}{0.0038240917782}{0.0200273330606}{0.0}{0.0427398492858}
\boxplotlabels{12}{0.0254284134881}{0.00922517220568}{0.0427398492858}{0.0038240917782}{0.0466801793502}
\boxplotlabels{16}{0.0335431540704}{0.0254284134881}{0.0427398492858}{0.0038240917782}{0.0466801793502}
\boxplotlabels{20}{0.0284768342445}{0.0254284134881}{0.0351907397237}{0.0038240917782}{0.0466801793502}
\boxplotlabels{24}{0.0300910291928}{0.0261686021612}{0.0350430114016}{0.0038240917782}{0.0430062101305}
\boxplotlabels{28}{0.0336094122626}{0.0293476635126}{0.0354946717749}{0.0038240917782}{0.0430062101305}
\boxplotlabels{32}{0.0353901389007}{0.0335307942436}{0.0370883100995}{0.0250598857564}{0.0430062101305}
\boxplotlabels{36}{0.0362512475452}{0.0341143734006}{0.0378396486085}{0.0324447636348}{0.0441711470976}
\boxplotlabels{40}{0.0374502613716}{0.0368629471041}{0.0397388884554}{0.0354304822378}{0.0448794307975}
\boxplotlabels{50}{0.0369708321747}{0.0368272558592}{0.038236571473}{0.034705901291}{0.0441711470976}
\boxplotlabels{60}{0.0443321206658}{0.0410096928639}{0.0463411824596}{0.034705901291}{0.0477377381606}
\boxplotlabels{70}{0.0432004569645}{0.0384471412976}{0.0449839850135}{0.034705901291}{0.0477377381606}
\boxplotlabels{80}{0.0422457859828}{0.0361027447074}{0.044935692943}{0.0304169659077}{0.046892822441}
\boxplotlabels{90}{0.0425415064847}{0.041907819695}{0.044935692943}{0.0389410969842}{0.046892822441}
\boxplotlabels{100}{0.0455131748664}{0.0450832258461}{0.046065966464}{0.0422899561354}{0.0474842634447}
\boxplotlabels{110}{0.0422899561354}{0.042121246204}{0.0458202813095}{0.0404903835339}{0.046892822441}
\boxplotlabels{120}{0.0422899561354}{0.0404903835339}{0.0422899561354}{0.0}{0.0452060684233}
\boxplotlabels{130}{0.0422899561354}{0.0}{0.0422899561354}{0.0}{0.0422899561354}
\boxplotlabels{140}{0.0}{0.0}{0.0}{0.0}{0.0}
\boxplotlabels{150}{0.157696102801}{0.0662089316418}{0.21479083733}{0.0}{0.224719101124}
\boxplotlabels{160}{0.175556220361}{0.142023208903}{0.238757330598}{0.0}{0.400850611377}
\boxplotlabels{170}{0.201864458729}{0.142023208903}{0.251748370207}{0.00266134397871}{0.510365251728}
\boxplotlabels{180}{0.203719393698}{0.150953267683}{0.252531577464}{0.00266134397871}{0.512567767373}
\boxplotlabels{190}{0.304234226928}{0.200758506772}{0.388475796371}{0.116687578419}{0.639927895448}
\boxplotlabels{200}{0.377374189476}{0.249630547647}{0.423048374846}{0.120225422668}{0.744707347447}
\boxplotlabels{210}{0.382855162855}{0.249630547647}{0.495267680086}{0.12375}{0.746268656716}
\boxplotlabels{220}{0.478841149713}{0.266325528342}{0.539589387962}{0.12375}{0.746268656716}
\boxplotlabels{230}{0.523542346649}{0.364007504587}{0.566993398863}{0.127261384903}{0.746268656716}
\boxplotlabels{240}{0.555271869059}{0.502426653043}{0.577404712636}{0.130759651308}{0.830174081238}
\boxplotlabels{250}{0.570250635984}{0.44815843546}{0.656199091091}{0.272727272727}{0.906926406926}
\boxplotlabels{260}{0.597327335496}{0.553355155483}{0.717425407854}{0.362350380849}{0.92039800995}
\boxplotlabels{270}{0.654382709121}{0.577645718845}{0.713200840102}{0.391366906475}{0.939249146758}
\boxplotlabels{280}{0.72570861267}{0.579255913542}{0.763160258565}{0.471873293282}{0.940334128878}
\boxplotlabels{290}{0.726390999897}{0.644132784892}{0.841750996552}{0.501449275362}{0.946440677966}
\boxplotlabels{300}{0.736457563118}{0.67068440821}{0.850625581154}{0.532084043157}{0.946119959336}
\boxplotlabels{310}{0.770014322525}{0.73415677805}{0.870062944457}{0.6060932866}{0.946440677966}
\boxplotlabels{320}{0.788488063928}{0.767124389043}{0.870062944457}{0.626826029216}{0.946440677966}
\boxplotlabels{330}{0.85525666303}{0.842148596145}{0.925857714218}{0.626826029216}{0.947652819993}
\boxplotlabels{340}{0.893057008344}{0.854241938186}{0.939493651325}{0.626826029216}{0.947652819993}
\boxplotlabels{350}{0.919819018848}{0.866776512684}{0.93101989546}{0.754296626353}{0.947652819993}
\boxplotlabels{360}{0.92979382493}{0.868293747722}{0.947264556408}{0.824129651861}{0.951585976628}
\boxplotlabels{370}{0.932358300569}{0.882279331738}{0.947434752971}{0.807743658211}{0.951585976628}
\boxplotlabels{380}{0.946876292822}{0.91561348004}{0.949731828774}{0.795601917113}{0.954183266932}
\boxplotlabels{390}{0.93883935651}{0.915693722601}{0.948760924066}{0.808013355593}{0.954183266932}
\boxplotlabels{400}{0.93883935651}{0.915693722601}{0.947409552842}{0.808013355593}{0.961949265688}
\boxplotlabels{410}{0.93883935651}{0.915693722601}{0.950922670346}{0.808013355593}{0.961949265688}
\boxplotlabels{420}{0.939015025871}{0.915693722601}{0.950922670346}{0.839024390244}{0.961949265688}
\boxplotlabels{430}{0.942892240605}{0.918941842691}{0.950922670346}{0.839024390244}{0.961949265688}
\boxplotlabels{440}{0.942856102332}{0.918941842691}{0.9522215091}{0.839024390244}{0.961949265688}
\boxplotlabels{450}{0.943730948621}{0.93182223397}{0.953749207217}{0.839024390244}{0.961949265688}
\boxplotlabels{460}{0.948020505115}{0.933062563361}{0.953749207217}{0.840909090909}{0.961949265688}
\boxplotlabels{470}{0.932021208289}{0.891109950448}{0.954470239609}{0.841232227488}{0.961949265688}
\boxplotlabels{480}{0.942483585065}{0.929305596509}{0.954470239609}{0.861607142857}{0.961949265688}
\boxplotlabels{490}{0.953589715461}{0.951932133926}{0.955374527344}{0.861607142857}{0.961152042867}
\boxplotlabels{500}{0.954153245175}{0.951932133926}{0.957693752112}{0.861607142857}{0.962864721485}
\boxplotlabels{510}{0.954153245175}{0.951932133926}{0.957693752112}{0.861518825782}{0.968085106383}
\boxplotlabels{520}{0.954153245175}{0.951924199791}{0.957693752112}{0.92800551154}{0.968085106383}
\boxplotlabels{530}{0.954153245175}{0.952411983146}{0.957693752112}{0.92800551154}{0.968085106383}
\boxplotlabels{540}{0.956208774532}{0.953271265909}{0.959560997127}{0.928881469115}{0.968085106383}
\boxplotlabels{550}{0.956208774532}{0.953271265909}{0.959362455184}{0.938693467337}{0.968085106383}
\boxplotlabels{560}{0.95616655382}{0.953271265909}{0.960680434127}{0.938693467337}{0.968085106383}
\boxplotlabels{570}{0.956327954404}{0.953271265909}{0.961006607202}{0.938652363393}{0.968085106383}
\boxplotlabels{580}{0.956501678979}{0.953271265909}{0.961818070534}{0.938652363393}{0.970257766028}
\boxplotlabels{590}{0.957013498208}{0.953271265909}{0.961818070534}{0.938652363393}{0.968428049186}
\boxplotlabels{600}{0.957707720739}{0.953271265909}{0.961818070534}{0.938652363393}{0.96875}
\boxplotlabels{610}{0.957974474734}{0.953271265909}{0.962209790614}{0.938652363393}{0.96875}
\boxplotlabels{620}{0.957974474734}{0.953497349955}{0.962503195485}{0.938652363393}{0.96875}
\boxplotlabels{630}{0.957974474734}{0.953497349955}{0.962503195485}{0.938652363393}{0.96875}
\boxplotlabels{640}{0.958146791842}{0.953497349955}{0.962705964958}{0.938652363393}{0.96875}
\boxplotlabels{650}{0.958146791842}{0.953497349955}{0.962705964958}{0.938652363393}{0.96875}
\boxplotlabels{660}{0.961119284294}{0.953763578693}{0.962705964958}{0.938652363393}{0.96875}
\boxplotlabels{670}{0.96127967109}{0.953763578693}{0.962705964958}{0.938652363393}{0.96875}
\boxplotlabels{680}{0.96127967109}{0.953755936774}{0.962840468626}{0.938652363393}{0.96875}
\boxplotlabels{690}{0.96127967109}{0.953755936774}{0.963048196182}{0.939008042895}{0.96875}
\boxplotlabels{700}{0.96127967109}{0.95356101856}{0.962949750782}{0.939008042895}{0.96875}
\boxplotlabels{710}{0.96127967109}{0.955145681391}{0.962949750782}{0.939008042895}{0.96875}
\boxplotlabels{720}{0.96127967109}{0.955352265959}{0.962949750782}{0.940073652494}{0.96875}
\boxplotlabels{730}{0.961093917138}{0.957047073046}{0.963187751446}{0.938926174497}{0.96875}
\boxplotlabels{740}{0.961310767298}{0.958112380484}{0.963187751446}{0.938926174497}{0.96875}
\boxplotlabels{750}{0.961659886455}{0.958112380484}{0.964462249847}{0.938926174497}{0.969435215947}
\boxplotlabels{760}{0.962393551763}{0.960521553247}{0.964444712025}{0.938926174497}{0.969435215947}
\boxplotlabels{770}{0.963799238068}{0.961515196838}{0.965408300173}{0.938926174497}{0.969435215947}
\boxplotlabels{780}{0.963799238068}{0.96168832071}{0.965488563104}{0.938926174497}{0.969435215947}
\boxplotlabels{790}{0.963799238068}{0.962377612011}{0.965328090609}{0.938926174497}{0.970822281167}
\boxplotlabels{800}{0.963799238068}{0.962377612011}{0.965328090609}{0.938926174497}{0.971466489715}
\boxplotlabels{810}{0.963799238068}{0.962639571899}{0.965723382082}{0.938926174497}{0.971466489715}
\boxplotlabels{820}{0.964177539609}{0.962639571899}{0.966533864542}{0.949230265313}{0.973745430376}
\fi


\addplot+[mark=triangle*] coordinates{(4,0.0128219547857)(8,0.0130028570951)(12,0.0262657243006)(16,0.0304431375945)(20,0.0274161796669)(24,0.0287037858294)(28,0.0314242301867)(32,0.0355193350448)(36,0.0370235085975)(40,0.0388643505741)(50,0.0380708457774)(60,0.0431477059544)(70,0.041814463556)(80,0.0406247272415)(90,0.0429315955313)(100,0.0452281732509)(110,0.0434023626249)(120,0.0378126999702)(130,0.0253739736813)(140,0.0)(150,0.134328719337)(160,0.187629149775)(170,0.221810542611)(180,0.226287087584)(190,0.310001867924)(200,0.354346031131)(210,0.381259077443)(220,0.422163791336)(230,0.462616312879)(240,0.526807708932)(250,0.560160376138)(260,0.612732899507)(270,0.647387960368)(280,0.692588065608)(290,0.728656092306)(300,0.751755299597)(310,0.785406943268)(320,0.813101975009)(330,0.848276840913)(340,0.865105212307)(350,0.891484001082)(360,0.908323281033)(370,0.907865561743)(380,0.913542893205)(390,0.916331505938)(400,0.916611576467)(410,0.917543097324)(420,0.920679334661)(430,0.922754025644)(440,0.923032962507)(450,0.934454507194)(460,0.935999937465)(470,0.919725275896)(480,0.931637016851)(490,0.943256210013)(500,0.944035475903)(510,0.944548682686)(520,0.951194177607)(530,0.951259215388)(540,0.954659413768)(550,0.955683428473)(560,0.956114370804)(570,0.956208942223)(580,0.957157360173)(590,0.956710011245)(600,0.956881050833)(610,0.957091089664)(620,0.957284857871)(630,0.957284857871)(640,0.957351033009)(650,0.957351033009)(660,0.957981028665)(670,0.958013106024)(680,0.958044448436)(690,0.958146733066)(700,0.958081365811)(710,0.958527767373)(720,0.958853312175)(730,0.958984344956)(740,0.959358750478)(750,0.959763052493)(760,0.960374813104)(770,0.961597705196)(780,0.961827285623)(790,0.962188742536)(800,0.962289442336)(810,0.962558376888)(820,0.964111856136)};
%\addlegendimage{mark=square,black}
%\addlegendentry{ED2}

%/home/neutatz/logs/out/features/labels_experiment_data_Movies_ActiveClean_time_1536888775.39.csv
\addplot+ coordinates{(4,0.0213699246429)(8,0.018672455839)(12,0.0212269210164)(16,0.0321859050029)(20,0.0302529715162)(24,0.0312966670441)(28,0.0329036450315)(32,0.0359456442243)(36,0.0362360527391)(40,0.0373720221553)(50,0.0365295786506)(60,0.0399637390442)(70,0.0396634157051)(80,0.0376468158517)(90,0.0401027864695)(100,0.0407462897094)(110,0.0400748188806)(120,0.0254856276499)(130,0.0211449780677)(140,0.0)(150,0.0966531273071)(160,0.141423326588)(170,0.179134219875)(180,0.223841111275)(190,0.29688743408)(200,0.312847885815)(210,0.344385073948)(220,0.385060993021)(230,0.416739663949)(240,0.451277478572)(250,0.465866659793)(260,0.483012177018)(270,0.506150957658)(280,0.539425530035)(290,0.590232006895)(300,0.59608046538)(310,0.618599698236)(320,0.644984383666)(330,0.66830500273)(340,0.672003120162)(350,0.68214825492)(360,0.703699482277)(370,0.719049704374)(380,0.720719668672)(390,0.730477562962)(400,0.746109009953)(410,0.759416318644)(420,0.767150779153)(430,0.785989994014)(440,0.792311304818)(450,0.803714154561)(460,0.808222165768)(470,0.816337660442)(480,0.824918607543)(490,0.828190598686)(500,0.833482001285)(510,0.847544471012)(520,0.852813587133)(530,0.849899107867)(540,0.869668106025)(550,0.87716977191)(560,0.885232740822)(570,0.889790242799)(580,0.891769033357)(590,0.8952894312)(600,0.899684410528)(610,0.901725438998)(620,0.905594719839)(630,0.909027750391)(640,0.911709521088)(650,0.914019773261)(660,0.916558038142)(670,0.921322370599)(680,0.92598281494)(690,0.928283325498)(700,0.929717395436)(710,0.930281349226)(720,0.931473600858)(730,0.933947004953)(740,0.935917181674)(750,0.936847890754)(760,0.937830161208)(770,0.938798513396)(780,0.940469627994)(790,0.94412115832)(800,0.945103480671)(810,0.945895549105)(820,0.947401733562)};
%\addlegendentry{ActiveClean Features}

\addplot+ coordinates{(4,0.0427398492858)(8,0.0254284134881)(12,0.0335431540704)(16,0.0377965937993)(20,0.0327689787002)(24,0.0331144608538)(28,0.0355431985121)(32,0.0373797858828)(36,0.0386114010969)(40,0.039813795573)(50,0.0385525870815)(60,0.042691476551)(70,0.0414795889613)(80,0.0398769660348)(90,0.0453044134093)(100,0.047776955024)(110,0.046892822441)(120,0.0452060684233)(130,0.0422899561354)(140,0.0)(150,0.124311172342)(160,0.152986519733)(170,0.163688294397)(180,0.193371335719)(190,0.213678902127)(200,0.283302065209)(210,0.293174935203)(220,0.320930640883)(230,0.363774601212)(240,0.387260784473)(250,0.401895832852)(260,0.40266659988)(270,0.414513006853)(280,0.416948256434)(290,0.444168796795)(300,0.46829440364)(310,0.485200425699)(320,0.508464072152)(330,0.524551017551)(340,0.532795964891)(350,0.549754775839)(360,0.556293913975)(370,0.552377964564)(380,0.54529269414)(390,0.528634622548)(400,0.543605333665)(410,0.567204079983)(420,0.5897479797)(430,0.56804840657)(440,0.55706787858)(450,0.554203263307)(460,0.551930542343)(470,0.533808865665)(480,0.504798058387)(490,0.488483557357)(500,0.474084543253)(510,0.474921374158)(520,0.511456999025)(530,0.492038474406)(540,0.498352924842)(550,0.484246401938)(560,0.496432040641)(570,0.503414551819)(580,0.503050330709)(590,0.512743732242)(600,0.517446385383)(610,0.500276959698)(620,0.497993788468)(630,0.501025810887)(640,0.500406805629)(650,0.504772573676)(660,0.559042914462)(670,0.537927160177)(680,0.527748450903)(690,0.530648437073)(700,0.514803846991)(710,0.518315693315)(720,0.486675662256)(730,0.504005835925)(740,0.483432588972)(750,0.499160668048)(760,0.494003208549)(770,0.516502506299)(780,0.472987561948)(790,0.458869978315)(800,0.485209712074)(810,0.470402388933)(820,0.461336332384)};
%\addlegendentry{BoostClean Features}


\addplot+[no marks, line width=2] coordinates{(0,0.027924399795675122)(801,0.027924399795675122)};
%\addlegendentry{KATARA}

\addplot+[no marks, line width=2] coordinates{(0,0.5978514712751051)(801,0.5978514712751051)};
%\addlegendentry{NADEEF}



%\addplot+[mark=x] coordinates{(0,0.3272573124205172)(801,0.3272573124205172)};
%\addlegendentry{Gaussian}
%\addplot+[mark=x] coordinates{(0,0.2267059623668102)(801,0.2267059623668102)};
%\addlegendentry{Histogram}
\addplot+[mark=x] coordinates{(0,0.34236856467163906)(801,0.342368564672)}; 
%\addlegendentry{Mixture}

\addplot coordinates{(0,0.0)(0,0.00)(10,0.12)(20,0.24)(30,0.28)(40,0.40)(50,0.40)(60,0.34)(70,0.34)(80,0.46)(90,0.41)(100,0.41)(110,0.43)(120,0.43)(130,0.37)(140,0.37)(150,0.37)(160,0.43)(170,0.43)(180,0.44)(190,0.44)(200,0.44)(210,0.49)(220,0.49)(230,0.44)(240,0.44)(250,0.44)(260,0.44)(270,0.44)(280,0.44)(290,0.43)(300,0.43)};
%\addlegendentry{Metadata Driven}






==> charts/model_all/address.tex <==
\nextgroupplot[legend to name=testLegendmodels, title={Address},
xmax=\limitaddress]
                
\addplot+[mark=none,ultra thick] coordinates{(4,4.45634571693e-05)(8,0.000533875772422)(12,0.00187224532449)(16,0.0880811560933)(20,0.214350161358)(24,0.297821127911)(28,0.321419012045)(38,0.345073985411)(48,0.380578140582)(58,0.406479428381)(68,0.367411225585)(78,0.569563254268)(88,0.528832189682)(98,0.679545268641)(108,0.723363921202)(118,0.855141253753)(128,0.9488082876)(138,0.961009819773)(148,0.978559413536)(158,0.981431957379)(168,0.977373149248)(178,0.981610169427)(188,0.981834763881)(198,0.982487837017)(208,0.981374839083)(218,0.978467430347)(228,0.979819719222)(238,0.98177073335)(248,0.981844905677)(258,0.982412319122)(268,0.984435084943)(278,0.984435411308)(288,0.985252684341)(298,0.985764530723)(308,0.98579617025)(318,0.987304720857)(328,0.987378561414)(338,0.986782950009)(348,0.988209042027)(358,0.987045905805)(368,0.987273881296)(378,0.98625337016)(388,0.988433174262)(398,0.990294883165)(408,0.991069527691)(418,0.99110075764)(428,0.991095635592)(438,0.990858042257)(448,0.991190170235)(458,0.991290897933)(468,0.991636946818)(478,0.991013330016)(488,0.991631606298)(498,0.991716520841)(508,0.991766351453)(518,0.991904536841)(528,0.992186374205)(538,0.99247272661)(548,0.992608802595)(558,0.992648735039)(568,0.992661577812)};
\addlegendentry{Tree Boosting}


\addplot+[mark=none,ultra thick] coordinates{(4,4.10433914936e-05)(8,0.000587220387513)(12,0.00228270140575)(16,0.0885331346135)(20,0.163255313181)(24,0.216643240613)(28,0.240066528536)(38,0.266785925643)(48,0.293270235029)(58,0.323429875344)(68,0.32338196844)(78,0.433758022424)(88,0.47441993908)(98,0.467539084139)(108,0.469482925953)(118,0.51613444614)(128,0.534571108213)(138,0.558823871945)(148,0.553553258505)(158,0.571520655479)(168,0.579087807479)(178,0.579773419418)(188,0.590023601238)(198,0.587085493127)(208,0.591429929581)(218,0.597889559826)(228,0.61167367007)(238,0.61486204149)(248,0.621275119508)(258,0.624402559002)(268,0.626961104912)(278,0.629495332034)(288,0.632855958181)(298,0.638294542291)(308,0.643208143928)(318,0.644947195625)(328,0.651386621197)(338,0.654972609445)(348,0.655644056553)(358,0.659503895931)(368,0.662588774386)(378,0.666198034897)(388,0.668019105376)(398,0.676863439113)(408,0.679279979856)(418,0.682169607807)(428,0.683020844123)(438,0.686693068964)(448,0.690852397113)(458,0.70049617239)(468,0.702658810973)(478,0.704827922188)(488,0.707967562243)(498,0.710495467716)(508,0.713354760975)(518,0.715869656376)(528,0.713816232853)(538,0.719171103497)(548,0.720614805389)(558,0.722829830683)(568,0.728588153733)};
\addlegendentry{Linear SVM}


\addplot+[mark=none,ultra thick] coordinates{(4,0.00010608324116)(8,0.000951629623228)(12,0.00335228548124)(16,0.133604381147)(20,0.320114318602)(24,0.406306225793)(28,0.430170754599)(38,0.458317435629)(48,0.487723360229)(58,0.533865489477)(68,0.531908143763)(78,0.544048884185)(88,0.557677229708)(98,0.563494541391)(108,0.574594061938)(118,0.58766452338)(128,0.590680278426)(138,0.592030501733)(148,0.600461671076)(158,0.602557790557)(168,0.604765551035)(178,0.609064293039)(188,0.609242454542)(198,0.612312293474)(208,0.61567109883)(218,0.619650919352)(228,0.621769798846)(238,0.623196371362)(248,0.623910856063)(258,0.626154750463)(268,0.633558268721)(278,0.636785541842)(288,0.637641637742)(298,0.636749126486)(308,0.638516839352)(318,0.639506747342)(328,0.640505049428)(338,0.640119129564)(348,0.640101916659)(358,0.640488559767)(368,0.641151469907)(378,0.641990340845)(388,0.641967846091)(398,0.641729780353)(408,0.642775224459)(418,0.643125164978)(428,0.643428197478)(438,0.643396289563)(448,0.644491385679)(458,0.645136063431)(468,0.64520208541)(478,0.645198796414)(488,0.639429383845)(498,0.640121715833)(508,0.640551756035)(518,0.64048504434)(528,0.640508576888)(538,0.640248045839)(548,0.640954908548)(558,0.640536973909)(568,0.640436680146)};
\addlegendentry{Naive Bayes}




==> charts/model_all/beers.tex <==
\nextgroupplot[title={Beers},
%ylabel={$F_1$-score},
xmax=\limitbeers]

\addplot+[mark=none,ultra thick] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(26,0.355747523108)(36,0.360915294744)(46,0.364017758745)(56,0.365024225466)(66,0.513546779872)(76,0.788256936715)(86,0.875355126852)(96,0.943880453182)(106,0.944558037082)(116,0.944786389388)(126,0.944874132476)(136,0.950390766524)(146,0.950450874548)(156,0.95081143732)(166,0.959296600138)(176,0.965375894461)(186,0.968738351438)(196,0.973957211721)(206,0.976757402121)(216,0.979273600257)(226,0.98076467162)(236,0.986352826695)(246,0.989633249975)(256,0.990976771431)(266,0.990976771431)(276,0.993830682963)(286,0.996774193548)(296,0.996774193548)(306,0.996774193548)(316,0.996774193548)(326,0.997127799736)(336,1.0)(346,1.0)(356,1.0)(366,1.0)(376,1.0)(386,1.0)(396,1.0)(406,1.0)(416,1.0)(426,1.0)(436,1.0)(446,1.0)};
%\addlegendentry{XGBOOST}


\addplot+[mark=none,ultra thick] coordinates{(4,0.202217062248)(8,0.313496856429)(12,0.261843852547)(16,0.235259834795)(26,0.196066265468)(36,0.205474856262)(46,0.241339938398)(56,0.294338403696)(66,0.241746603415)(76,0.25025307259)(86,0.253554712151)(96,0.296355929951)(106,0.34692771538)(116,0.382836522812)(126,0.445716890719)(136,0.484671029078)(146,0.523881076923)(156,0.548915200649)(166,0.57275342873)(176,0.595733770191)(186,0.604286335449)(196,0.659513518114)(206,0.687246221989)(216,0.700285497532)(226,0.660567063379)(236,0.745462994692)(246,0.766491219425)(256,0.836719154911)(266,0.856139427325)(276,0.881912733657)(286,0.910801410414)(296,0.915295509884)(306,0.930022778176)(316,0.932189944561)(326,0.934519161204)(336,0.938082799981)(346,0.94021819242)(356,0.944632390333)(366,0.948573012061)(376,0.949611598214)(386,0.953472401738)(396,0.955523335141)(406,0.95804459196)(416,0.959261316932)(426,0.961664004189)(436,0.962945799441)(446,0.965011933611)};
%\addlegendentry{Linear SVM}


\addplot+[mark=none,ultra thick] coordinates{(4,0.224369536086)(8,0.502742447379)(12,0.481253201538)(16,0.448802464255)(26,0.43538085284)(36,0.226555786126)(46,0.218441641228)(56,0.208323194532)(66,0.20429205692)(76,0.221315291008)(86,0.216225570246)(96,0.230431906311)(106,0.236786496641)(116,0.249698899479)(126,0.267635833025)(136,0.283070173185)(146,0.297871389429)(156,0.306298128595)(166,0.3246574081)(176,0.340720446779)(186,0.35491810131)(196,0.371429078113)(206,0.37889861458)(216,0.388547859674)(226,0.407134455785)(236,0.416360157451)(246,0.429246162222)(256,0.43314337338)(266,0.446049033289)(276,0.454536501167)(286,0.467365187686)(296,0.476179738183)(306,0.482599154327)(316,0.482505458868)(326,0.487918355834)(336,0.493947096878)(346,0.501511256932)(356,0.509863288296)(366,0.525089535598)(376,0.531048397373)(386,0.541537574737)(396,0.545662795508)(406,0.549228106419)(416,0.55051405763)(426,0.553518040004)(436,0.558833567403)(446,0.561979084705)};
%\addlegendentry{Multinomial Naive Bayes}




==> charts/model_all/flights.tex <==
\nextgroupplot[title={Flights},
ylabel={$F_1$-score},
xmax=\limitflights]

\addplot+[mark=none,ultra thick] coordinates{(4,0.124862938596)(8,0.288525613817)(12,0.394081957887)(16,0.484588379916)(26,0.601117448274)(36,0.675424531498)(46,0.730183553516)(56,0.807274269262)(66,0.815323932721)(76,0.824312276919)(86,0.833625034305)(96,0.84386446802)(106,0.849791057706)(116,0.856702092297)(126,0.869380968093)(136,0.878308953786)(146,0.886006070873)(156,0.893181199057)(166,0.899003302149)(176,0.902715562919)(186,0.912571934185)(196,0.91843659323)(206,0.925564440052)(216,0.929644715409)(226,0.934140236101)(236,0.938678899152)(246,0.942315951184)(256,0.945887895748)(266,0.948046311707)(276,0.95099462801)(286,0.953069367404)};
%\addlegendentry{XGBOOST}


\addplot+[mark=none,ultra thick] coordinates{(4,0.0719406731181)(8,0.28169647267)(12,0.332655907538)(16,0.415742375109)(26,0.527798623413)(36,0.572561994151)(46,0.629274023741)(56,0.647375062598)(66,0.662668476896)(76,0.709883001455)(86,0.715126176721)(96,0.743292746941)(106,0.778292490649)(116,0.786693579152)(126,0.799449763057)(136,0.812573774067)(146,0.822443991765)(156,0.833756804651)(166,0.832646467175)(176,0.844317674506)(186,0.847878324495)(196,0.852475638492)(206,0.853799031776)(216,0.862162358607)(226,0.867488126961)(236,0.875861141155)(246,0.880068211356)(256,0.88339564129)(266,0.889843958119)(276,0.892159386626)(286,0.895066051058)}; 
%\addlegendentry{Linear SVM}


\addplot+[mark=none,ultra thick] coordinates{(4,0.231114459251)(8,0.439024607047)(12,0.567906618498)(16,0.65934968822)(26,0.63750435699)(36,0.689221480134)(46,0.676227455633)(56,0.690920506948)(66,0.693560790998)(76,0.699616385038)(86,0.698225397845)(96,0.702365022741)(106,0.706613711036)(116,0.712480734141)(126,0.715579140455)(136,0.720378391196)(146,0.722510222888)(156,0.724625359958)(166,0.728567172583)(176,0.729841839458)(186,0.731836244624)(196,0.731631365509)(206,0.733975765606)(216,0.734496947102)(226,0.736055679064)(236,0.736207164015)(246,0.738235893787)(256,0.738419599992)(266,0.739556653084)(276,0.740656620453)(286,0.741215382344)};
%\addlegendentry{Multinomial Naive Bayes}




==> charts/model_all/movies.tex <==
\nextgroupplot[title={Movies},
%ylabel={$F_1$-score},
xmax=\limitmovies]

\addplot+[mark=none,ultra thick] coordinates{(4,0.0213699246429)(8,0.0177061306149)(12,0.0283179610083)(16,0.0317197618294)(20,0.0294938033561)(24,0.0301636697569)(28,0.0341835724816)(32,0.0361861248933)(36,0.0370010576614)(40,0.0384361401485)(50,0.0368770959058)(60,0.0415625850836)(70,0.0401958790563)(80,0.0382771798369)(90,0.043957869876)(100,0.0454083103389)(110,0.0359847109789)(120,0.0340552728456)(130,0.0253739736813)(140,0.0)(150,0.0776274823475)(160,0.170684523472)(170,0.264019526658)(180,0.320697627846)(190,0.393224037158)(200,0.453147235117)(210,0.516040547437)(220,0.549976906899)(230,0.574241686501)(240,0.586161883463)(250,0.639531773723)(260,0.698645312762)(270,0.74102926933)(280,0.783213793304)(290,0.800624763244)(300,0.820788417378)(310,0.840924322869)(320,0.860147157825)(330,0.901885510038)(340,0.90796912239)(350,0.920275110134)(360,0.920814084026)(370,0.928134657667)(380,0.928134657667)(390,0.935412939409)(400,0.935325673362)(410,0.9386120947)(420,0.941187139753)(430,0.930360312702)(440,0.93222709206)(450,0.935006041435)(460,0.926217031786)(470,0.926033021343)(480,0.926845162455)(490,0.941418194155)(500,0.951920736735)(510,0.95246871992)(520,0.953089914918)(530,0.953014364467)(540,0.953689369799)(550,0.955030734782)(560,0.955129976463)(570,0.956067763646)(580,0.95323029608)(590,0.954582658431)(600,0.958233838787)(610,0.961488994093)(620,0.961486699088)(630,0.96151852432)(640,0.950458689392)(650,0.963739734489)(660,0.963946797982)(670,0.964135042534)(680,0.964232295326)(690,0.964758447255)(700,0.965445340688)(710,0.965308216373)(720,0.96578276484)(730,0.965990045905)(740,0.966507803594)(750,0.966537368326)(760,0.967063503616)(770,0.96737053007)(780,0.96797635429)(790,0.968042080629)(800,0.968042080629)(810,0.968042080629)(820,0.968074309806)};
%\addlegendentry{XGBOOST}


\addplot+[mark=none,ultra thick] coordinates{(4,0.0314465156063)(8,0.0134558470796)(12,0.0161637550816)(16,0.0182514988538)(20,0.0181253389415)(24,0.0172405800975)(28,0.015686030494)(32,0.0144687428441)(36,0.014963870561)(40,0.015696947418)(50,0.0218814365713)(60,0.0251492100936)(70,0.0351061543927)(80,0.0432728622682)(90,0.0461915719662)(100,0.0627294197908)(110,0.0974856996295)(120,0.148425874987)(130,0.22848217755)(140,0.405599760217)(150,0.412932226754)(160,0.429410224013)(170,0.499623133797)(180,0.526551975986)(190,0.549946611423)(200,0.582843778952)(210,0.595419062663)(220,0.616087030328)(230,0.623644985106)(240,0.651000927027)(250,0.658991752043)(260,0.666280327888)(270,0.686007881285)(280,0.69412671876)(290,0.700671287836)(300,0.711093177268)(310,0.71692976001)(320,0.727648423697)(330,0.70623782822)(340,0.711233937169)(350,0.716390243428)(360,0.723423532897)(370,0.735120976649)(380,0.739880163663)(390,0.743606905729)(400,0.744025906662)(410,0.745406135038)(420,0.741573103632)(430,0.747390060704)(440,0.754880572035)(450,0.752965845172)(460,0.758787540247)(470,0.767353056742)(480,0.773984713551)(490,0.782664289913)(500,0.785484185896)(510,0.790583428299)(520,0.792837458607)(530,0.794653176137)(540,0.796565062816)(550,0.797593743684)(560,0.797892161339)(570,0.796364416589)(580,0.798116249565)(590,0.798720773367)(600,0.804102128337)(610,0.816794749468)(620,0.829462520143)(630,0.827142109811)(640,0.83188416349)(650,0.835530132331)(660,0.83567866516)(670,0.836560982016)(680,0.837767155885)(690,0.835261271895)(700,0.843326192408)(710,0.846194511071)(720,0.846491777519)(730,0.844779299049)(740,0.850778791652)(750,0.851387816388)(760,0.852318874914)(770,0.852806076252)(780,0.855476189496)(790,0.856315329492)(800,0.857303644552)(810,0.858150584381)(820,0.857929857579)};
%\addlegendentry{Linear SVM}


\addplot+[mark=none,ultra thick] coordinates{(4,0.118704031261)(8,0.0660529803235)(12,0.0813848687871)(16,0.100847371215)(20,0.0806639595734)(24,0.0848842342934)(28,0.0922412950078)(32,0.101181511228)(36,0.107004641444)(40,0.111699777724)(50,0.112209576394)(60,0.127158303108)(70,0.13912841489)(80,0.146105332925)(90,0.18152709173)(100,0.208549028814)(110,0.236157978589)(120,0.284480048721)(130,0.366687606575)(140,0.531614894658)(150,0.520148913935)(160,0.577615397879)(170,0.597680470023)(180,0.620494937849)(190,0.633830390221)(200,0.628540024931)(210,0.65791053946)(220,0.674568687311)(230,0.679974824243)(240,0.700255182903)(250,0.71147895988)(260,0.714911573772)(270,0.732023918769)(280,0.746672888397)(290,0.753750562753)(300,0.768393709939)(310,0.772497603103)(320,0.767453595824)(330,0.791777735214)(340,0.791026574275)(350,0.801513303774)(360,0.805430901529)(370,0.801044079557)(380,0.812514879571)(390,0.79548901106)(400,0.809985479762)(410,0.814889045245)(420,0.825495447316)(430,0.824018390089)(440,0.836071708201)(450,0.835300492209)(460,0.828773693102)(470,0.839857056317)(480,0.846287797224)(490,0.843671932532)(500,0.849245928203)(510,0.851067103177)(520,0.845612603867)(530,0.848679793618)(540,0.852284550877)(550,0.853340391121)(560,0.855787605391)(570,0.858235990301)(580,0.85882588508)(590,0.8611098978)(600,0.860414598839)(610,0.860410031013)(620,0.854199306784)(630,0.859892687372)(640,0.85972652684)(650,0.860418060798)(660,0.863447994012)(670,0.867745057499)(680,0.868231276108)(690,0.864052710827)(700,0.869779574589)(710,0.870022455079)(720,0.87085030587)(730,0.872468737081)(740,0.872127431752)(750,0.872784333439)(760,0.873131937538)(770,0.873472055467)(780,0.87461722147)(790,0.874511274001)(800,0.87487806516)(810,0.875710112122)(820,0.876013260479)};
%\addlegendentry{Multinomial Naive Bayes}




==> charts/order_all/address.tex <==
\nextgroupplot[legend to name=testLegendorder,
title={Address},
%ylabel={$F_1$-score},
xmin=0.0, xmax=\limitaddress]
                
\addplot+[mark=none] coordinates{(4,5.57043214617e-05)(8,0.000770131313035)(12,0.00258981673248)(16,0.0761495003703)(20,0.175006337204)(24,0.264270158576)(28,0.300285413506)(38,0.334525872174)(48,0.37960710205)(58,0.419816516404)(68,0.393184072361)(78,0.574541660862)(88,0.531939168201)(98,0.683455776853)(108,0.75991041799)(118,0.835520570216)(128,0.901719664236)(138,0.954807818214)(148,0.974378773945)(158,0.976456412918)(168,0.977810099187)(178,0.977526223595)(188,0.977789784894)(198,0.97918458833)(208,0.979005029974)(218,0.979850247544)(228,0.983238043903)(238,0.985393627225)(248,0.976763947524)(258,0.98544140125)(268,0.985280201349)(278,0.985829274018)(288,0.986500154704)(298,0.987617837884)(308,0.983155114088)(318,0.984627938379)(328,0.986972726229)(338,0.988813264942)(348,0.988060586867)(358,0.988062203895)(368,0.98879832559)(378,0.988854496017)(388,0.98867251495)(398,0.989645033356)(408,0.989787060881)(418,0.989979834727)(428,0.990023853161)(438,0.99013276516)(448,0.990263165219)(458,0.990112714178)(468,0.990322009701)(478,0.990324897267)(488,0.990435445146)(498,0.991137663201)(508,0.991570978924)(518,0.991715991982)(528,0.992076573078)(538,0.992520205565)(548,0.9925814222)(558,0.993223067917)(568,0.993228192589)};
\addlegendentry{Min Certainty (MC)}


\addplot+[mark=none] coordinates{(4,6.6845185754e-05)(8,0.000571007432637)(12,0.00225813502786)(16,0.0914457692439)(20,0.216239885773)(24,0.263873018727)(28,0.294013095172)(38,0.328865872429)(48,0.367855098024)(58,0.40449064494)(68,0.371541035302)(78,0.546240988987)(88,0.538220960738)(98,0.6854616973)(108,0.702033987093)(118,0.732636358553)(128,0.765381023089)(138,0.799496157357)(148,0.817272963606)(158,0.859200001663)(168,0.868020712366)(178,0.906913927132)(188,0.920930866817)(198,0.939533444776)(208,0.964417295092)(218,0.964190459047)(228,0.96639844991)(238,0.978714279851)(248,0.980221474365)(258,0.98022702236)(268,0.979554503848)(278,0.980935353959)(288,0.98692408336)(298,0.988927770811)(308,0.988625477741)(318,0.988916759716)(328,0.988892548524)(338,0.988700617006)(348,0.98905679107)(358,0.989064008039)(368,0.989085260833)(378,0.989107770161)(388,0.989119910614)(398,0.989120102546)(408,0.98913124835)(418,0.989128504619)(428,0.989140550111)(438,0.98914830748)(448,0.98915116189)(458,0.989155028045)(468,0.989158593908)(478,0.989156095758)(488,0.989168310217)(498,0.989184429218)(508,0.989168337925)(518,0.989190394976)(528,0.989195204571)(538,0.989201620528)(548,0.989207790502)(558,0.989202067445)(568,0.989212670266)};
\addlegendentry{Max Prediction Change (MPC)}


\addplot+[mark=none] coordinates{(4,6.6845185754e-05)(8,0.000571007432637)(12,0.00225813502786)(16,0.0914457692439)(20,0.216239885773)(24,0.263873018727)(28,0.294013095172)(38,0.328865872429)(48,0.367855098024)(58,0.40449064494)(68,0.376263513136)(78,0.547868140917)(88,0.544787132919)(98,0.69117323595)(108,0.691174867998)(118,0.691178590613)(128,0.691182215397)(138,0.840203034648)(148,0.836901574361)(158,0.960299184703)(168,0.961852111226)(178,0.961855068184)(188,0.961826056126)(198,0.961832504182)(208,0.954493451901)(218,0.967915666887)(228,0.964964326183)(238,0.964964326183)(248,0.96496701774)(258,0.96502633869)(268,0.965023086181)(278,0.955873881141)(288,0.959121063774)(298,0.959577985544)(308,0.959577985544)(318,0.959582364715)(328,0.959628868082)(338,0.959910745624)(348,0.971492475373)(358,0.972828476343)(368,0.982739933377)(378,0.982739933377)};
\addlegendentry{Round-Robin (RR)}


\addplot+[mark=none, thick, dash dot] coordinates{(4,0.0625456079132)(8,0.112065256067)(12,0.156455835318)(22,0.138877295909)(32,0.107520779687)(36,0.133235824921)(46,0.20503635866)(56,0.269823618407)(66,0.33204577885)(70,0.412302287008)(80,0.424864071022)(90,0.456416831048)(100,0.558145775841)(110,0.590804478775)(120,0.579663091326)(130,0.640810982877)(140,0.662946024531)(144,0.658823946269)(148,0.700626387416)(158,0.711926941476)(168,0.750344453163)(178,0.764546413045)(188,0.795956251012)(198,0.799222394281)(208,0.834416605996)(218,0.87436832412)(228,0.896213516226)(238,0.91165066355)(248,0.925181644441)(258,0.926487459113)(268,0.92480395029)(278,0.92533514663)(288,0.9227764957)(298,0.936632023147)(308,0.958580568338)(318,0.960578160091)(328,0.961563221286)(338,0.958397876558)(348,0.958399849332)(358,0.959349071232)(368,0.958786217236)(378,0.9637400163)(388,0.986333437382)(398,0.986693542299)(408,0.986977541321)(418,0.989095682512)(428,0.987989666594)(438,0.987894750981)(448,0.98948160955)(458,0.989359026517)(468,0.989432909557)(478,0.989641055338)(488,0.99041430888)(498,0.99024216809)(508,0.990598029222)(518,0.990329884079)(528,0.990484004867)(538,0.990501734613)(548,0.990580938695)(558,0.991048617376)(568,0.991100503445)(578,0.990679746428)(588,0.990694106468)(598,0.99067749983)(608,0.991198860243)(618,0.991314271178)(628,0.99149321102)(638,0.991495824581)(648,0.991539495801)(658,0.991931896032)(668,0.99192705756)};
\addlegendentry{Random (RA)}


\addplot+[mark=none, thick, dash dot] coordinates{(4,6.6845185754e-05)(8,0.000571007432637)(12,0.00225813502786)(16,0.0914457692439)(20,0.216239885773)(24,0.263873018727)(28,0.294013095172)(38,0.328865872429)(48,0.367855098024)(58,0.40449064494)(68,0.364648937115)(78,0.539532373764)(88,0.533017165349)(98,0.680732782158)(108,0.680732782158)(118,0.680734455196)(128,0.680743795377)(138,0.680747715772)(148,0.680751616263)(158,0.680760444103)(168,0.680754739552)(178,0.680804739834)(188,0.680819139762)(198,0.680824314703)(208,0.697114663053)(218,0.707461673751)(228,0.725171102036)(238,0.771211285381)(248,0.811832739746)(258,0.826497075253)(268,0.82658766093)(278,0.84181795982)(288,0.86791035126)(298,0.912392399465)(308,0.93173600766)(318,0.937054398825)(328,0.937126235498)(338,0.932518310234)(348,0.932529748707)(358,0.926840600383)(368,0.926892339188)(378,0.927348842571)(388,0.932805690461)(398,0.930503004751)(408,0.953682034078)(418,0.966911947178)(428,0.968409169995)(438,0.968451041826)(448,0.968444523322)(458,0.968003524892)(468,0.968532121515)(478,0.968549096696)(488,0.968551812207)(498,0.968554188162)(508,0.968509516811)(518,0.968575287674)(528,0.96859803687)(538,0.968706664738)(548,0.968755037638)(558,0.968756688191)(568,0.968765063409)};
\addlegendentry{Max Error (ME)}


==> charts/order_all/beers.tex <==
\nextgroupplot[title={Beers},
ylabel={$F_1$-score},
xmin=0.0, xmax=\limitbeers]
                
\addplot+[mark=none] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(26,0.355747523108)(36,0.360915294744)(46,0.364017758745)(56,0.365024225466)(66,0.513546779872)(76,0.788256936715)(86,0.875355126852)(96,0.943880453182)(106,0.944558037082)(116,0.944786389388)(126,0.944874132476)(136,0.950390766524)(146,0.950450874548)(156,0.95081143732)(166,0.959296600138)(176,0.965375894461)(186,0.968738351438)(196,0.973957211721)(206,0.976757402121)(216,0.979273600257)(226,0.98076467162)(236,0.986352826695)(246,0.989633249975)(256,0.990976771431)(266,0.990976771431)(276,0.993830682963)(286,0.996774193548)(296,0.996774193548)(306,0.996774193548)(316,0.996774193548)(326,0.997127799736)(336,1.0)(346,1.0)(356,1.0)(366,1.0)(376,1.0)(386,1.0)(396,1.0)(406,1.0)(416,1.0)(426,1.0)(436,1.0)(446,1.0)};
%\addlegendentry{Min certainty (MC)}


\addplot+[mark=none] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(26,0.239919199266)(36,0.247729227719)(46,0.249333951937)(56,0.250901387789)(66,0.538923470273)(76,0.56463719979)(86,0.742708885962)(96,0.893778850654)(106,0.900897670443)(116,0.909178769216)(126,0.925933591497)(136,0.932643281812)(146,0.959412558038)(156,0.975453745538)(166,0.976736188988)(176,0.986550172094)(186,0.986550172094)(196,0.986550172094)(206,0.986550172094)(216,0.986550172094)(226,0.986550172094)(236,0.986550172094)(246,0.986550172094)(256,0.986550172094)(266,0.986550172094)(276,0.986550172094)(286,0.986550172094)(296,0.986550172094)(306,0.986550172094)(316,0.986550172094)(326,0.986550172094)(336,0.986550172094)(346,0.986550172094)(356,0.986550172094)(366,0.986550172094)(376,0.986550172094)(386,0.986550172094)(396,0.986550172094)(406,0.986550172094)(416,0.986550172094)(426,0.986550172094)(436,0.986550172094)(446,0.986550172094)};
%\addlegendentry{Max prediction change (MPC)}


\addplot+[mark=none] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(26,0.244853143496)(36,0.254913201498)(46,0.255841381765)(56,0.257349099727)(66,0.533850261277)(76,0.776219148589)(86,0.79131086256)(96,0.797838884012)(106,0.797838884012)(116,0.948145128504)(126,0.953764198724)(136,0.961813679271)(146,0.961813679271)(156,0.961813679271)(166,0.979682978917)(176,0.988470820428)(186,0.988470820428)(196,0.988470820428)(206,0.988470820428)(216,0.994795172574)};
%\addlegendentry{Round-robin (RR)}


\addplot+[mark=none] coordinates{(4,0.0)(8,0.0046046046046)(18,0.00583191227881)(22,0.0867971124019)(26,0.138481768142)(36,0.202390851706)(46,0.363617498096)(56,0.432362219945)(66,0.504848036348)(76,0.69272323673)(86,0.711150339712)(96,0.889616807414)(106,0.903053814257)(116,0.903996163618)(126,0.905509895183)(136,0.918351911427)(146,0.921615916016)(156,0.925655210786)(166,0.936001302086)(176,0.936001302086)(186,0.972644163405)(196,0.976753225345)(206,0.977008653225)(216,0.976650952053)(226,0.976650952053)(236,0.976896273723)(246,0.979839205582)(256,0.983414780576)(266,0.983594405929)(276,0.983594405929)(286,0.983594405929)(296,0.985335797958)(306,0.98673839536)(316,0.989394193415)(326,0.996883254094)(336,0.996883254094)(346,0.996883254094)(356,0.996883254094)(366,0.996883254094)(376,0.998014629049)(386,0.998014629049)(396,0.998014629049)(406,0.998014629049)(416,0.998014629049)(426,1.0)(436,1.0)(446,1.0)(456,1.0)(466,1.0)(476,1.0)(486,1.0)(496,1.0)(506,1.0)(516,1.0)(526,1.0)(536,1.0)(546,1.0)(556,1.0)(566,1.0)};
%\addlegendentry{Random (RA)}


\addplot+[mark=none] coordinates{(4,0.0)(8,0.0)(12,0.0)(16,0.0)(26,0.243672838653)(36,0.251533020404)(46,0.252188985816)(56,0.25379486623)(66,0.277701368)(76,0.313290774032)(86,0.340963181532)(96,0.397266158515)(106,0.462145812222)(116,0.613291411324)(126,0.735252129748)(136,0.840657550071)(146,0.930443116593)(156,0.974879233417)(166,0.989461134955)(176,0.989461134955)(186,0.989461134955)(196,0.999017071909)(206,0.999017071909)(216,0.999017071909)(226,0.999017071909)(236,0.999017071909)(246,0.999017071909)(256,0.999017071909)(266,0.999017071909)(276,0.999017071909)(286,0.999017071909)(296,0.999017071909)(306,0.999017071909)(316,0.999017071909)(326,0.999017071909)(336,0.999017071909)(346,0.999017071909)(356,0.999017071909)(366,0.999017071909)(376,0.999017071909)(386,0.999017071909)(396,0.999017071909)(406,0.999017071909)(416,0.999017071909)(426,0.999017071909)(436,0.999017071909)(446,0.999017071909)};
%\addlegendentry{Max error (ME)}


==> charts/order_all/flights.tex <==
\nextgroupplot[title={Flights},
ylabel={$F_1$-score},
xmin=0.0, xmax=\limitflights]
                
\addplot+[mark=none] coordinates{(4,0.174808114035)(8,0.295762455923)(12,0.396196265773)(16,0.488310733565)(26,0.593472088167)(36,0.686717721195)(46,0.734377258196)(56,0.787735034815)(66,0.807734607929)(76,0.822575395328)(86,0.83269145929)(96,0.846267222307)(106,0.86054513197)(116,0.871938396169)(126,0.881360293616)(136,0.886764005995)(146,0.894667172177)(156,0.906847993689)(166,0.910121065962)(176,0.915354155589)(186,0.918875753539)(196,0.924078738366)(206,0.927862461545)(216,0.932168248625)(226,0.935302616591)(236,0.940198595218)(246,0.941935833797)(256,0.943772821041)(266,0.945489556424)(276,0.948097400636)(286,0.948780246342)};
%\addlegendentry{Min certainty (MC)}


\addplot+[mark=none] coordinates{(4,0.149835526316)(8,0.339580204388)(12,0.393021288285)(16,0.510849667677)(26,0.613014674335)(36,0.677116835135)(46,0.728467281664)(56,0.788114090446)(66,0.785978324904)(76,0.795202104984)(86,0.807424661298)(96,0.817612726532)(106,0.837855633307)(116,0.852786229427)(126,0.865737980663)(136,0.878038350784)(146,0.884782970191)(156,0.892255548967)(166,0.899862484436)(176,0.907518931959)(186,0.912699669608)(196,0.919296753745)(206,0.928198303541)(216,0.934579090124)(226,0.937309986003)(236,0.941818336291)(246,0.945340565387)(256,0.948609974821)(266,0.951732966342)(276,0.952949173818)(286,0.955778979897)};
%\addlegendentry{Max prediction change (MPC)}


\addplot+[mark=none] coordinates{(4,0.149835526316)(8,0.339580204388)(12,0.393021288285)(16,0.510849667677)(26,0.613718723167)(36,0.681076453108)(46,0.732202004529)(56,0.786549659627)(66,0.786720696206)(76,0.786141651043)(86,0.812638328085)(96,0.810607887146)(106,0.81344668744)(116,0.822719790318)(126,0.846222609818)(136,0.871540478141)(146,0.872264538452)(156,0.881606530861)(166,0.891988082809)(176,0.900666997674)(186,0.900944137)(196,0.906815467896)(206,0.915517894849)(216,0.922404797152)};
%\addlegendentry{Round-robin (RR)}


\addplot+[mark=none, thick, dash dot] coordinates{(4,0.225328947368)(8,0.315559853758)(12,0.389357159021)(22,0.481683624924)(32,0.532669741602)(42,0.587847267057)(52,0.652150872004)(62,0.688154919804)(72,0.711956857156)(82,0.733578401365)(86,0.739141514844)(96,0.759792636231)(106,0.789626322652)(116,0.797934237004)(126,0.829446024272)(136,0.840620211024)(146,0.848187830638)(156,0.855538846986)(166,0.857718658245)(176,0.866752268847)(186,0.877728411052)(196,0.887788233328)(206,0.897499067428)(216,0.906686830156)(226,0.910444191026)(236,0.915008371583)(246,0.919323680622)(256,0.923195110585)(266,0.926327640649)(276,0.92943676348)(286,0.932285113704)(296,0.935765775757)(306,0.937264557293)(316,0.937581659173)(326,0.93997660753)};
%\addlegendentry{Random (RA)}


\addplot+[mark=none, thick, dash dot] coordinates{(4,0.149835526316)(8,0.339580204388)(12,0.393021288285)(16,0.510849667677)(26,0.61377249604)(36,0.678504484186)(46,0.730427775135)(56,0.787837140642)(66,0.78803767094)(76,0.79959855049)(86,0.817609587047)(96,0.825186070426)(106,0.836792135373)(116,0.841898954444)(126,0.860645676894)(136,0.876297258313)(146,0.885812231153)(156,0.89608405787)(166,0.899187879468)(176,0.904552137945)(186,0.906344995297)(196,0.911165762203)(206,0.915042524767)(216,0.917298689027)(226,0.919128491813)(236,0.92155106239)(246,0.923139713893)(256,0.92499738798)(266,0.926394240406)(276,0.927594419313)(286,0.929513016966)};
%\addlegendentry{Max error (ME)}


==> charts/order_all/movies.tex <==
\nextgroupplot[title={Movies},
%ylabel={$F_1$-score},
xmin=0.0, xmax=\limitmovies]
                
\addplot+[mark=none] coordinates{(4,0.0341918794286)(8,0.0276497142874)(12,0.0318037195359)(16,0.0329111969282)(20,0.0276330065822)(24,0.0282642184562)(28,0.0352771308471)(32,0.0369852545497)(36,0.0380800969031)(40,0.0391433604189)(50,0.0370306581367)(60,0.0405408008074)(70,0.0397241374339)(80,0.0373830823835)(90,0.0406254459191)(100,0.0418030736262)(110,0.0402158737002)(120,0.0341669268143)(130,0.0211449780677)(140,0.0)(150,0.0912632170429)(160,0.123937238749)(170,0.203627773916)(180,0.273319805706)(190,0.335073039134)(200,0.350746526699)(210,0.423147890656)(220,0.475329196743)(230,0.498856629035)(240,0.572537603181)(250,0.637588760445)(260,0.654677560418)(270,0.696872674316)(280,0.734466410621)(290,0.767975578839)(300,0.792723146875)(310,0.808363943469)(320,0.8347592077)(330,0.871064158369)(340,0.902938361189)(350,0.921862078151)(360,0.930638604841)(370,0.93182443004)(380,0.943702776533)(390,0.945500669729)(400,0.947596414011)(410,0.948210651338)(420,0.946636486754)(430,0.950435521875)(440,0.951073420619)(450,0.947711252143)(460,0.933222474576)(470,0.944734997518)(480,0.94700377147)(490,0.950355577115)(500,0.953020632773)(510,0.953460809754)(520,0.955510079625)(530,0.955298521578)(540,0.955172832876)(550,0.943622567879)(560,0.956800951992)(570,0.957395595852)(580,0.957388737061)(590,0.958070670133)(600,0.957935481554)(610,0.959665708758)(620,0.959994834957)(630,0.961341492132)(640,0.961829388736)(650,0.962171525355)(660,0.962401708222)(670,0.963065624119)(680,0.96316304128)(690,0.963400647307)(700,0.963308072932)(710,0.966175894307)(720,0.966275690368)(730,0.966892471759)(740,0.966985796594)(750,0.96707361628)(760,0.967073830574)(770,0.967944601451)(780,0.967978375188)(790,0.968299952506)(800,0.969014651095)(810,0.969848054659)(820,0.970249875377)};
%\addlegendentry{Min certainty (MC)}


\addplot+[mark=none] coordinates{(4,0.0170959397143)(8,0.0134321456863)(12,0.0258103752443)(16,0.0290720773194)(20,0.0274908289845)(24,0.0297127150342)(28,0.0343911934006)(32,0.0364037637317)(36,0.0381112886616)(40,0.0394725187098)(50,0.0387484525404)(60,0.0435389547524)(70,0.0425694180043)(80,0.04129452517)(90,0.0454758031662)(100,0.0466464698261)(110,0.0449276506018)(120,0.0429165292701)(130,0.0296029692948)(140,0.0)(150,0.134489913099)(160,0.153399212784)(170,0.23395948143)(180,0.328943232976)(190,0.372170773744)(200,0.453319345653)(210,0.481967711638)(220,0.501901761512)(230,0.517291088107)(240,0.54783610225)(250,0.586446264315)(260,0.600388611739)(270,0.632006691868)(280,0.649920901454)(290,0.647964970111)(300,0.66008470843)(310,0.662833744229)(320,0.663335280917)(330,0.673018022248)(340,0.675091091145)(350,0.678497971136)(360,0.679623092123)(370,0.680249370412)(380,0.691148658502)(390,0.6918885607)(400,0.699606898756)(410,0.710359702335)(420,0.710554654203)(430,0.71085395148)(440,0.711148751361)(450,0.723839884399)(460,0.732200183908)(470,0.732289497909)(480,0.732459913356)(490,0.732459913356)(500,0.732490518453)(510,0.732490518453)(520,0.732490518453)(530,0.732490518453)(540,0.732490518453)(550,0.732490518453)(560,0.732490518453)(570,0.732490518453)(580,0.732490518453)(590,0.732490518453)(600,0.732490518453)(610,0.732490518453)(620,0.732490518453)(630,0.732490518453)(640,0.732490518453)(650,0.732490518453)(660,0.732490518453)(670,0.732490518453)(680,0.732490518453)(690,0.732490518453)(700,0.732490518453)(710,0.732490518453)(720,0.732490518453)(730,0.732490518453)(740,0.732490518453)(750,0.732490518453)(760,0.732490518453)(770,0.732490518453)(780,0.732490518453)(790,0.732490518453)(800,0.732490518453)(810,0.732490518453)(820,0.732490518453)};
%\addlegendentry{Max prediction change (MPC)}


\addplot+[mark=none] coordinates{(4,0.0213699246429)(8,0.0207860085966)(12,0.0266595335963)(16,0.0340300183757)(20,0.0323758254106)(24,0.0309705262151)(28,0.0346905199355)(32,0.0383888699108)(36,0.0403719080475)(40,0.0406202759868)(50,0.0400232181294)(60,0.0425047343349)(70,0.0419804143671)(80,0.040787023954)(90,0.0452435055093)(100,0.0464088761063)(110,0.0451668205933)(120,0.0419050890007)(130,0.0126869868406)(140,0.0)(150,0.127065264259)(160,0.12812189658)(170,0.204954554536)(180,0.268459660106)(190,0.272399282184)(200,0.292261237531)(210,0.38540434133)(220,0.466251231505)(230,0.514879177045)(240,0.582115843273)(250,0.632215085862)(260,0.632991311307)(270,0.689009140037)(280,0.757732176391)(290,0.757837470501)(300,0.775175888987)(310,0.798270216156)(320,0.835271720863)(330,0.834258771788)(340,0.857613624117)(350,0.861658117966)(360,0.861869853873)(370,0.864051188668)(380,0.864051188668)(390,0.866621894675)(400,0.871609480068)(410,0.879271528412)(420,0.880016197063)(430,0.930622025365)(440,0.937791918727)(450,0.937791918727)(460,0.938422838471)(470,0.942608448718)(480,0.942608448718)(490,0.947043518015)(500,0.948688887524)(510,0.953761556087)(520,0.953786680134)(530,0.95196512018)(540,0.955342936151)};
%\addlegendentry{Round-robin (RR)}


\addplot+[mark=none, thick, dash dot] coordinates{(4,0.0170959397143)(8,0.0289410079368)(12,0.0258653650747)(16,0.0281785232077)(26,0.0299918139541)(30,0.0436521473447)(34,0.0391163235689)(44,0.0483332671249)(54,0.0488570459033)(58,0.0444923280132)(68,0.0478044626869)(78,0.0516887328949)(88,0.0549374887147)(92,0.0533350355344)(102,0.0525486312058)(112,0.0497733566057)(122,0.0540943893497)(126,0.0778753901439)(136,0.086784793246)(146,0.0922349797533)(150,0.137495839853)(160,0.107181979116)(170,0.109602592057)(180,0.137147131249)(190,0.146170681414)(200,0.185901380224)(210,0.191750984499)(220,0.220424509009)(230,0.26956367556)(240,0.289627749416)(250,0.29821605672)(260,0.306254651779)(270,0.307318363938)(280,0.364912338127)(290,0.368769433246)(300,0.440063128576)(310,0.440351198989)(320,0.488658075518)(330,0.612551378505)(340,0.656995661422)(350,0.684021021579)(360,0.71652645058)(370,0.773775029767)(380,0.79903082469)(390,0.800148772022)(400,0.8223497281)(410,0.837409750075)(420,0.846579841006)(430,0.85503873556)(440,0.855736820702)(450,0.851255147549)(460,0.871285887032)(470,0.883488828109)(480,0.893011100562)(490,0.893112469217)(500,0.89513245671)(510,0.902616771509)(520,0.914180169086)(530,0.915191739555)(540,0.914624497335)(550,0.918618621785)(560,0.915416990246)(570,0.915448769708)(580,0.918948974545)(590,0.917835192449)(600,0.917647554289)(610,0.918910010896)(620,0.920290680137)(630,0.927842034142)(640,0.928241247365)(650,0.929810522571)(660,0.929721347473)(670,0.929875611256)(680,0.931581223985)(690,0.931588483935)(700,0.931936621903)(710,0.94136242819)(720,0.941564872893)(730,0.885698862339)(740,0.886454214771)(750,0.948572417129)(760,0.948753089246)(770,0.955365289296)(780,0.955826462675)(790,0.968982791821)(800,0.969351762279)(810,0.969782011909)(820,0.970754180908)(830,0.971085141092)(840,0.971682710126)(850,0.972069079561)(860,0.972597788838)(870,0.972836140218)(880,0.973993130794)(890,0.974515775276)(900,0.974549481294)(910,0.975158674971)(920,0.975353295211)(930,0.972415942567)(940,0.972415942567)(950,0.974271443807)(960,0.974399734332)};
%\addlegendentry{Random (RA)}


\addplot+[mark=none, thick, dash dot] coordinates{(4,0.0170959397143)(8,0.0134321456863)(12,0.0258103752443)(16,0.0290720773194)(20,0.0274908289845)(24,0.0297127150342)(28,0.0343911934006)(32,0.0364037637317)(36,0.0381112886616)(40,0.0394725187098)(50,0.0387484525404)(60,0.0435389547524)(70,0.0425694180043)(80,0.04129452517)(90,0.0454758031662)(100,0.0466464698261)(110,0.0449276506018)(120,0.0429165292701)(130,0.0296029692948)(140,0.0)(150,0.105487686059)(160,0.19317127924)(170,0.195568454727)(180,0.210988765773)(190,0.213837607959)(200,0.243123839927)(210,0.250010140358)(220,0.267951587457)(230,0.290914648043)(240,0.308059696778)(250,0.343606806718)(260,0.3813395724)(270,0.370128349016)(280,0.385167130669)(290,0.39605480715)(300,0.432078436881)(310,0.475208908665)(320,0.481639757326)(330,0.51034889254)(340,0.541770975175)(350,0.548894730829)(360,0.572889925368)(370,0.574385983751)(380,0.586616464507)(390,0.589899187919)(400,0.600225464139)(410,0.616681402479)(420,0.624194785234)(430,0.645961753663)(440,0.665019208354)(450,0.671260171269)(460,0.680619917157)(470,0.684255419086)(480,0.684255419086)(490,0.68437165239)(500,0.684558950687)(510,0.684634763512)(520,0.684634763512)(530,0.68467346152)(540,0.684709587219)(550,0.696465666153)(560,0.710371356442)(570,0.710408145433)(580,0.710708045758)(590,0.711081240945)(600,0.720781222309)(610,0.734372693444)(620,0.74007412791)(630,0.748695829797)(640,0.760606214896)(650,0.774884157264)(660,0.779563591944)(670,0.787091181147)(680,0.802194193889)(690,0.80232455171)(700,0.806142719766)(710,0.806142719766)(720,0.806142719766)(730,0.806142719766)(740,0.806142719766)(750,0.806142719766)(760,0.806142719766)(770,0.806142719766)(780,0.806142719766)(790,0.806142719766)(800,0.806142719766)(810,0.806142719766)(820,0.806142719766)};
%\addlegendentry{Max error (ME)}


==> tables/runtime_table_fancy.tex <==
\begin{table}[t]
	\centering
	\caption{Runtime (seconds) of the error detection results presented in Table~\ref{tab:effectivity}.}
	\label{tab:runtime}
	\resizebox{\columnwidth}{!}{
		\begin{tabular}{@{}lrcrcrcr@{}}\toprule
		Method
		& Flights 
		%& Citations 
		&& Movies 
		%&& Restaurants 
		&& Beers 
		&& Address 
		%&& Hospital 
		%& Salaries 
		\\ \midrule
		
		\system & 
		90 && %flights
		% & %citations
		670 && %movies
		%1,304 && %restaurants
		251 && %beers 336
		739 %address
		%690   %hospital
		%& 764 %Salaries
		\\ 
		
		ActiveClean 
		& 43 %flights
		%&  %citations
		&& 3,647 %movies
		%&& 3,694 %restaurants
		&& 468 %beers
		&& 5,914 %address
		%&& 354 %hospital
		%&  %Salaries
		\\ 
		
		BoostClean 
		& 81 %flights
		%&  %citations
		&& 589 %movies
		%&& 474 %restaurants
		&& 159 %beers
		&& 537 %address
		%&& 533 %hospital
		%&  %Salaries
		\\ 
		
		dBoost
		& 11 %flights
		%& x %citations
		&& 89 %movies
		%&& 88 %restaurants
		&& 4 %beers
		&& 536 %address
		%&& 4 %hospital
		%& x %Salaries
		\\
		 
		\iffalse
		Gaussian 
		& 2 %flights
		%& 2 %citations
		&& 24 %movies
		%&& 80 %restaurants
		&& 3 %beers
		&& 158 %address
		%&& 4 %hospital
		%& 293 %Salaries
		\\
		
		Histogram 
		& 2 %flights
		%& 2 %citations
		&& 27 %movies
		%&& 88 %restaurants
		&& 4 %beers
		&& 185  %address
		%&& 4 %hospital
		%& 372 %Salaries
		\\
		
		Mixture 
		& 11 %flights
		%& 17 %citations
		&& 89 %movies
		%&& 363 %restaurants
		&& 38 %beers
		&& 536 %address
		%&& 30 %hospital
		%& 5097 %Salaries
		\\ 
		
		\fi
		
		KATARA 
		& 83 %flights
		%& - %citations
		&& 608 %movies
		%&& 1,810 %restaurants
		&& 115 %beers
		&& 2,700 %address
		%&& 156 %hospital
		%& - %Salaries
		\\ 
		
		NADEEF 
		& 16 %flights
		%& 14 %citations
		&& 18 %movies
		%&& 0 %restaurants
		&& 16 %beers
		&& 46 %address 
		%&& 16 %hospital
		%& 14 %Salaries
		\\ 
		\bottomrule
		
		\end{tabular}
	}
\vspace{-5mm}
\end{table}

